PennyGS: Full Resolution 3DGS Training in Minutes on Consumer GPUs

3D Gaussian Splatting is increasingly fed by high-resolution captures from commodity devices, yet training still happens at reduced resolution with research-grade GPUs. We present PennyGS, a method to achieve full-resolution (4K) training of 3DGS on consumer GPUs by improving the efficiency of every stage of a training step. Improvements include a leaner splat with flat RGB color and a directional cone opacity, fused projection and key emission, forward rasterization optimizations with strided pixel sampling, an approximate tile SSIM loss, a warp-per-splat backward rasterization, and a fused backward projection and sparse Adam step. At the standard 30k-step budget, PennyGS is the fastest of 10 methods on Mip-NeRF 360 and Tanks&Temples 4K on all four GPUs at competitive quality, at least 3.9x faster than the quickest of the others, while peaking below 2 GB of GPU memory. On an RTX 3060, a full-resolution Mip-NeRF 360 scene trains in 6m 25s, faster than any other method trains it on an RTX 4090.

==> diagrams/cone_panel.tex <==
% Left panel of fig_alt_cone.tex (cone opacity geometry), for use inside tikzpicture[dg]. Copied 2026-11-14.
  \tikzset{lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute},
           cam/.style={circle, draw=dgink, line width=0.4pt, inner sep=0pt, minimum size=1.5mm},
           ray/.style={->, draw=dgink, line width=0.45pt, >={Latex[length=1.1mm, width=0.9mm]}}}
  % ---- left: geometry
  \node[lab, anchor=west] at (0,0) {\textbf{Visible only inside its cone}};
  \begin{scope}[shift={(2.05,-1.95)}, scale=0.88]
    \def\R{1.65}
    \foreach \i in {0,...,19} {
      \pgfmathsetmacro{\pa}{3*\i}
      \pgfmathsetmacro{\pb}{3*\i+3}
      \pgfmathsetmacro{\g}{40*(1-2*(1-cos(3*\i+1.5)))}
      \fill[black!\g] (0,0) -- (90-\pb:\R) arc (90-\pb:90-\pa:\R) -- cycle;
      \fill[black!\g] (0,0) -- (90+\pa:\R) arc (90+\pa:90+\pb:\R) -- cycle;
    }
    \draw[dgmute, line width=0.3pt, densely dotted] (150:\R) arc (150:390:\R);
    \draw[dgink, line width=0.4pt] (0,0) -- (30:\R) (0,0) -- (150:\R);
    \draw[dgink, line width=0.4pt] (30:\R) arc (30:150:\R);
    \draw[dgink, line width=0.3pt] (30:0.5) arc (30:90:0.5);
    \node[lab] at (60:0.68) {$60^\circ$};
    \draw[flow] (0,0) -- (90:1.12) node[above=1pt, lab] {$n$};
    \draw[ray] (0,0) -- (120:1.55);
    \node[lab] at (128:1.08) {$w$};
    \fill[dgink, rotate=15] (0,0) ellipse (0.12 and 0.055);
    \foreach \a/\f in {80/.97, 120/.73, 55/.64} {
      \node[cam, fill=dgink] at (\a:\R) {};
      \node[lab] at (\a:1.92) {$\f$};
    }
    \foreach \a in {180, 235, 325} \node[cam, fill=white] at (\a:\R) {};
  \end{scope}
  % key under the picture (2026-11-14), level with the spawn panel's key
  \node[cam, fill=dgink] at (0.17,-3.64) {};
  \node[lab, anchor=north west] at (0.4,-3.55) {sees it; number = opacity factor};
  \node[cam, fill=white] at (0.17,-3.92) {};
  \node[mut, anchor=north west] at (0.4,-3.83) {outside the cone: dropped};


==> diagrams/fig_alt_cone_p1.tex <==
% Left panel of fig_alt_cone.tex only (figure board pick 2026-11-13: "Visible only inside its cone").
% The full two-panel figure stays in fig_alt_cone.tex as the board's source.
% Claude's cone figure (2026-11-12), single column, no equations in the figure.
% Left: k = 2 cone (60 deg). The shading is the factor itself, f = 1 - 2 (1 - cos phi), drawn in 3-degree strips
% out to the camera circle, so the falloff reaches the edge where the cameras sit. Seen cameras at 10/30/35 deg
% from n -> f = 0.97 / 0.73 / 0.64; unseen at 90/145/125 deg off axis.
% Right: factor against viewing angle for k = 1, 1.75, 3.5, 6 and base splats (k <= 0): f = max(0, 1 - k (1 - cos theta)),
% zero beyond arccos(1 - 1/k) = 90, 64.6, 44.4, 33.6 deg.
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \tikzset{lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute},
           cam/.style={circle, draw=dgink, line width=0.4pt, inner sep=0pt, minimum size=1.5mm},
           ray/.style={->, draw=dgink, line width=0.45pt, >={Latex[length=1.1mm, width=0.9mm]}}}
  % ---- left: geometry
  \node[lab, anchor=west] at (0,0) {\textbf{Visible only inside its cone}};
  \begin{scope}[shift={(2.05,-2.15)}]
    \def\R{1.65}
    \foreach \i in {0,...,19} {
      \pgfmathsetmacro{\pa}{3*\i}
      \pgfmathsetmacro{\pb}{3*\i+3}
      \pgfmathsetmacro{\g}{40*(1-2*(1-cos(3*\i+1.5)))}
      \fill[black!\g] (0,0) -- (90-\pb:\R) arc (90-\pb:90-\pa:\R) -- cycle;
      \fill[black!\g] (0,0) -- (90+\pa:\R) arc (90+\pa:90+\pb:\R) -- cycle;
    }
    \draw[dgmute, line width=0.3pt, densely dotted] (150:\R) arc (150:390:\R);
    \draw[dgink, line width=0.4pt] (0,0) -- (30:\R) (0,0) -- (150:\R);
    \draw[dgink, line width=0.4pt] (30:\R) arc (30:150:\R);
    \draw[dgink, line width=0.3pt] (30:0.5) arc (30:90:0.5);
    \node[lab] at (60:0.68) {$60^\circ$};
    \draw[flow] (0,0) -- (90:1.12) node[above=1pt, lab] {$n$};
    \draw[ray] (0,0) -- (120:1.55);
    \node[lab] at (128:1.08) {$w$};
    \fill[dgink, rotate=15] (0,0) ellipse (0.12 and 0.055);
    \foreach \a/\f in {80/.97, 120/.73, 55/.64} {
      \node[cam, fill=dgink] at (\a:\R) {};
      \node[lab] at (\a:1.92) {$\f$};
    }
    \foreach \a in {180, 235, 325} \node[cam, fill=white] at (\a:\R) {};
  \end{scope}

\end{tikzpicture}
\caption{\textbf{Cone opacity.} Left: a splat with axis $n$ and slope $k=2$, whose cone reaches $60^\circ$; the shading is the opacity factor. Cameras outside the cone do not see the splat, so projection drops it before key emission. Right: the factor against angle for several $k$. Base splats keep a factor of 1.}
\Description{Left: a splat with axis n pointing up and a cone of 60 degrees whose shading fades from dark along n to white at the edge, reaching the circle of cameras. Three filled cameras on the cone's rim are labelled 0.97, 0.73 and 0.64; one has a ray w drawn to it. Three hollow cameras sit outside the cone on a dotted circle. Right: opacity factor against the angle from n, a flat line at 1 for base splats and four curves for varying k, each labelled along its slope, reaching zero at angles between 34 and 90 degrees.}
\label{fig:alt-cone}
\end{figure}


==> diagrams/fig_alt_cone_spawn.tex <==
% Cone opacity + cone spawn side by side in one column (board variant 2026-11-14).
% Left = cone_panel.tex (fig_alt_cone left panel), right = spawn_panel.tex (one-panel spawn).
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \useasboundingbox (0,0.15) rectangle (8.4,-4.35);
  \begin{scope}
    \input{diagrams/cone_panel}
  \end{scope}
  \begin{scope}[shift={(4.3,0)}]
    \input{diagrams/spawn_panel}
  \end{scope}
\end{tikzpicture}
\caption{\textbf{Cone opacity and cone spawn.} Left: a splat with axis $n$ and slope $k=2$, whose cone reaches $60^\circ$; the shading is the opacity factor. Cameras outside the cone do not see the splat, so projection drops it before key emission. Right: each splat counts, in every view, the high-error pixels it covers. When those views are much more concentrated than all views that see it, it gains a copy whose cone faces them; the original stays. Counts are illustrative.}
\Description{Left: a splat with axis n pointing up and a cone of 60 degrees whose shading fades from dark along n to white at the edge. Three filled cameras inside the cone are labelled 0.97, 0.73 and 0.64; three hollow cameras sit outside it. A key below explains filled and hollow cameras. Right: a splat inside a light full circle, with arrows all around it, each labelled with a number; five arrows in the upper middle are black and labelled 4, 15, 26, 18 and 7, the others grey and labelled 0 to 0.7. A shaded cone covers the black arrows: a new copy of the splat, visible only inside it, drawn on top of the original.}
\label{fig:alt-cone-spawn}
\end{figure}


==> diagrams/fig_alt_spawn.tex <==
% Claude's spawn figure (2026-11-12), single column, no equations.
% Views slightly uneven (user: neither too even nor too dense): grey at 0, 25, 45, 135, 158, 180; error views at
% 62, 78, 92, 105, 120 (~15 deg apart vs 20-25 for the rest). Number at each arrow = high-error pixels the splat covers
% in that view, per megapixel (FastGS measure, GS-CUDA kernels_densify.cu: pixel L1 error min-max rescaled over the
% image, high-error if > 0.1 (fastgs_loss_thresh); count_contrib counts masked pixels the splat contributes to with
% alpha >= 1/255; fastgs_accumulate: c_norm = count * 1e6 / pixels, direction added unweighted if c_norm >= 1).
% Values are a DEMO (consistent with the rule, not measured). 5 error views (the minimum the rule needs):
% r_e = 0.939 (mean axis 91.4 deg), r_c (all 11) = 0.628; 1 - r_e = 0.061 < 0.5 (1 - r_c) = 0.186 -> spawn;
% k = 1 / (2 (1 - r_e) + 0.25) = 2.68, child cone half-angle arccos(1 - 1/k) = 51 deg.
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \tikzset{lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute},
           ray/.style={->, draw=dgink, line width=0.55pt, >={Latex[length=1.1mm, width=0.9mm]}},
           gray ray/.style={ray, draw=black!35, line width=0.45pt},
           lead/.style={draw=dgmute, line width=0.3pt}}
  \useasboundingbox (0,0.15) rectangle (8.4,-3.95);
  % ---- 1: views with their error counts
  \node[lab, anchor=west] at (0,0) {\textbf{1\ \ Identify high-error view angles}};
  \begin{scope}[shift={(2.0,-2.35)}]
    \foreach \a/\v in {0/0, 25/0.3, 45/0.7, 135/0.5, 158/0.2, 180/0} {
      \draw[gray ray] (0,0) -- (\a:1.3);
      \node[mut] at (\a:1.58) {\v};
    }
    \foreach \a/\v in {62/4, 78/15, 92/26, 105/18, 120/7} {
      \draw[ray] (0,0) -- (\a:1.3);
      \node[lab] at (\a:1.55) {\v};
    }
    \fill[dgink, rotate=15] (0,0) ellipse (0.12 and 0.055);
  \end{scope}
  \node[lab, anchor=north west] at (0,-2.62) {1.\ count pixels with high L1 error};
  \node[lab, anchor=north west] at (0,-2.9) {2.\ identify views with many such pixels};
  \node[lab, anchor=north west] at (0,-3.18) {3.\ keep track of such view angles};

  % ---- 2: cone child next to the unchanged base splat
  \node[lab, anchor=west] at (4.55,0) {\textbf{2\ \ Add a cone child}};
  \begin{scope}[shift={(6.5,-1.55)}]
    \fill[black!7] (0,0) circle (1.05);
    \draw[dgmute, line width=0.3pt, densely dotted] (0,0) circle (1.05);
    \fill[black!26] (0,0) -- (40:1.05) arc (40:142:1.05) -- cycle;
    \draw[dgink, line width=0.4pt] (0,0) -- (40:1.05) (0,0) -- (142:1.05);
    \draw[flow] (0,0) -- (91:0.82);
    \fill[black!40, rotate=15] (-0.07,-0.05) ellipse (0.12 and 0.055);
    \fill[dgink, rotate=15] (0.07,0.05) ellipse (0.12 and 0.055);
  \end{scope}
  \fill[black!26] (4.55,-2.72) rectangle ++(0.22,-0.16);
  \node[lab, anchor=north west] at (4.85,-2.62) {child: a copy, opacity 0.1,};
  \node[lab, anchor=north west] at (4.85,-2.9) {cone toward the error views};
  \fill[black!7] (4.55,-3.35) rectangle ++(0.22,-0.16);
  \draw[dgmute, line width=0.3pt, densely dotted] (4.55,-3.35) rectangle ++(0.22,-0.16);
  \node[mut, anchor=north west] at (4.85,-3.25) {base: kept, seen from every view};
\end{tikzpicture}
\caption{\textbf{Cone spawn.} Each splat counts, in every view, the high-error pixels it covers. When those views are much more concentrated than all views that see it, it gains a copy whose cone faces them; the original stays. Counts are illustrative.}
\Description{Left: a splat with eleven arrows over 180 degrees, slightly closer together in the middle, each labelled with a number; the five middle arrows are black and labelled 4, 15, 26, 18 and 7, the others grey and labelled 0 to 0.7. Right: two overlapping splats at the same place, a light disc around them for the base splat visible from all sides, and a darker cone facing up for the child.}
\label{fig:alt-spawn}
\end{figure}


==> diagrams/fig_alt_spawn_one.tex <==
% Cone spawn as one panel (board variant 2026-11-14). Picture in spawn_panel.tex.
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \useasboundingbox (0,0.15) rectangle (4.1,-4.35);
  \input{diagrams/spawn_panel}
\end{tikzpicture}
\caption{\textbf{Cone spawn.} Each splat counts, in every view, the high-error pixels it covers. When those views are much more concentrated than all views that see it, it gains a copy whose cone faces them; the original stays. Counts are illustrative.}
\Description{A splat with eleven arrows over 180 degrees, each labelled with a number. The five middle arrows are black and labelled 4, 15, 26, 18 and 7; the others are grey and labelled 0 to 0.7. A shaded cone covers the five black arrows: a new copy of the splat, drawn on top of the original, is visible only inside it.}
\label{fig:alt-spawn}
\end{figure}


==> diagrams/fig_cone_failure.tex <==
% generated by figsrc/build_cone_failure.py -- do not edit
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{0.6pt}\renewcommand{\arraystretch}{0.4}
\begin{tabular}{@{}cc@{}}
  \includegraphics[width=\dimexpr(\linewidth-1.2pt)/2\relax]{figures/failure/Ignatius_sh2.jpg} &
  \includegraphics[width=\dimexpr(\linewidth-1.2pt)/2\relax]{figures/failure/Ignatius_ours.jpg} \\
  \includegraphics[width=\dimexpr(\linewidth-1.2pt)/2\relax]{figures/failure/Family_sh2.jpg} &
  \includegraphics[width=\dimexpr(\linewidth-1.2pt)/2\relax]{figures/failure/Family_ours.jpg} \\
  \sffamily\footnotesize SH degree 2 & \sffamily\footnotesize Ours (directional opacity) \\
\end{tabular}
% CAPTION (hand-edited, kept when the table is regenerated) begin
\caption[Failure cases of directional opacity]{Failure cases of directional opacity.\ {\normalfont
Artifacts are more extreme when they do appear in views far from training set.}}
% old: \caption{\textbf{Failure cases of directional opacity.}}
% CAPTION end
\Description{Two rows of paired renders from viewpoints away from the training cameras: the Ignatius statue and the Family statue. Left, a model with SH degree 2 renders both cleanly. Right, our model shows a bright glowing streak over the Ignatius statue and dark smears floating over the Family scene.}
\label{fig:cone_failure}
\end{figure}


==> diagrams/fig_mech_loss_inria_p1.tex <==
% Step 1 of fig_mech_loss_inria.tex only, one column: the panel picked on the figure board (2026-11-13).
% The full four-step figure stays in fig_mech_loss_inria.tex as the board's source.
% Loss in the original 3DGS with the current fused-ssim (rahul-goel/fused-ssim a7c48d6 ssim.cu) + PyTorch L1/autograd.
% fusedssimCUDA: 16x16 threads, per channel stages a 26x26 tile (5-pixel halo) of both images (sTile[26][26][2]),
% horizontal pass of 5 maps into xconv[26][16][5] (13 728 B shared), vertical pass; writes ssim_map + dm_dmu1,
% dm_dsigma1_sq, dm_dsigma12. fusedssim_backwardCUDA: per channel stages dL_dmap times each derivative map over 26x26
% (sData[3][26][26]), 3 blurs, writes dL_dimg1. L1 = abs().mean() in PyTorch; autograd sums the two gradients.
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \def\pstep#1#2#3#4{%
    \node[circle, draw=dgink, line width=0.4pt, fill=white, text=dgink, font=\sffamily\scriptsize\bfseries,
          inner sep=0pt, minimum size=3.1mm] at (#2+0.155,#3) {#1};
    \node[anchor=west, inner sep=0pt, text=dgink] at (#2+0.4,#3) {\textbf{#4}};}
  \tikzset{cell/.style={draw=dgink, line width=0.35pt, fill=white},
           lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute}}


  % --- 1: tiles and the haloed buffer (cell 0.05 cm = 1 pixel, tile = 16 px, buffer = 26 px)
  \node[anchor=west, inner sep=0pt, text=dgink] at (0,0) {\textbf{Stage a $26{\times}26$ buffer per tile}};
  \draw[black!14, line width=0.1pt, step=0.05] (0,-2.9) grid (2.4,-0.5);
  \draw[dgmute, line width=0.4pt, step=0.8] (0,-2.9) grid (2.4,-0.5);
  \fill[black, fill opacity=0.10] (0.55,-1.05) rectangle (1.85,-2.35);
  \fill[black, fill opacity=0.18] (0.8,-1.3) rectangle (1.6,-2.1);
  \draw[dgink, line width=0.5pt, dash pattern=on 2pt off 1.4pt] (0.55,-1.05) rectangle (1.85,-2.35);
  \draw[dgink, line width=0.8pt] (0.8,-1.3) rectangle (1.6,-2.1);
  \fill[black, fill opacity=0.45] (0.55,-1.05) rectangle (1.1,-1.6);
  \node[lab, anchor=west] at (2.6,-0.62) {block = tile:};
  \node[lab, anchor=west] at (2.6,-0.86) {256 threads};
  \node[mut, anchor=west] at (2.6,-1.25) {dashed: $26{\times}26$};
  \node[mut, anchor=west] at (2.6,-1.49) {staged, 2.6$\times$};
  \node[mut, anchor=west] at (2.6,-1.73) {the tile};
  \node[mut, anchor=west] at (2.6,-2.12) {dark: one};
  \node[mut, anchor=west] at (2.6,-2.36) {$11{\times}11$ window};
  \node[mut, anchor=west] at (0,-3.1) {Every pixel's window reaches 5 pixels out, so both};
  \node[mut, anchor=west] at (0,-3.35) {images are staged with a halo, one channel at a time.};

\end{tikzpicture}
\caption{\textbf{Loss in the original 3DGS} with fused-ssim, one block. (1) The block stages its tile and a 5-pixel halo of both images, $26\times26$ pixels. (2) It blurs five maps per channel with the $11\times11$ Gaussian window. (3) SSIM and its derivatives go to global memory; PyTorch forms the loss, and L1 runs separately. (4) A second kernel blurs the derivatives into the SSIM gradient.}
\Description{A few 16 by 16 tiles with their pixels; one tile's block stages a 26 by 26 buffer around it. Five maps per channel are blurred with an 11-tap Gaussian. The SSIM map and three derivative maps go to global memory, PyTorch computes the loss, and a second kernel reloads and blurs the derivative maps into the SSIM gradient, which autograd adds to the L1 gradient.}
\label{fig:mech-loss-inria}
\end{figure}


==> diagrams/fig_qualitative.tex <==
% generated by figsrc/build_qualitative.py -- do not edit
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{0.6pt}\renewcommand{\arraystretch}{0.4}
\providecommand{\qlab}[2]{\begin{tikzpicture}[baseline=(i.base)]\node[inner sep=0pt](i){#1};\node[anchor=south west, inner sep=1.2pt, fill=white, fill opacity=0.8, text opacity=1, font=\sffamily\scriptsize] at (i.south west) {#2};\end{tikzpicture}}
\begin{tabular}{@{}ccccc@{}}
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/garden_10_vksplat.jpg}}{48m\,16s, 26.10\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/garden_10_litegs.jpg}}{31m\,07s, 26.32\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/garden_10_lichtfeld.jpg}}{42m\,54s, 26.31\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/garden_10_ours.jpg}}{7m\,06s, 26.36\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/garden_10_gt.jpg}}{\itshape garden} \\
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bonsai_15_vksplat.jpg}}{15m\,45s, 31.77\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bonsai_15_litegs.jpg}}{16m\,01s, 32.87\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bonsai_15_lichtfeld.jpg}}{21m\,12s, 32.74\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bonsai_15_ours.jpg}}{2m\,33s, 32.81\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bonsai_15_gt.jpg}}{\itshape bonsai} \\
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bicycle_04_vksplat.jpg}}{36m\,55s, 23.81\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bicycle_04_litegs.jpg}}{32m\,07s, 24.64\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bicycle_04_lichtfeld.jpg}}{33m\,26s, 24.66\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bicycle_04_ours.jpg}}{6m\,29s, 24.35\,dB} &
  \qlab{\includegraphics[width=\dimexpr(\textwidth-4pt)/5\relax]{figures/qual/bicycle_04_gt.jpg}}{\itshape bicycle} \\
  \sffamily\footnotesize VkSplat & \sffamily\footnotesize LiteGS & \sffamily\footnotesize LichtFeld & \sffamily\footnotesize \textbf{Ours} & \sffamily\footnotesize Ground truth \\
\end{tabular}
% CAPTION (hand-edited, kept when the table is regenerated) begin
\caption[Qualitative comparison on held-out views]{Qualitative comparison on held-out views.\ {\normalfont
Crops of held-out views of Mip-NeRF~360 (garden, bonsai, bicycle). Each crop gives the method's training time on an RTX 3070 and its PSNR on that scene, as in \cref{tab:main_comparison}.}}
% old: \caption{\textbf{Qualitative comparison on held-out views.}}
% CAPTION end
\Description{A grid of image crops: three rows of held-out views (garden, bonsai, bicycle) and 5 columns (VkSplat, LiteGS, LichtFeld, ours, ground truth). Each crop is labelled with the method's training time on an RTX 3070 and its PSNR on that scene.}
\label{fig:qualitative}
\end{figure*}


==> diagrams/fig_quality_curve.tex <==
% Held-out PSNR (left: sampling, half-res training) and SSIM (right: loss, splat model) against training time (RTX 3070, mean over 15 scenes,
% 5k checkpoints, last = 30k). Plot generated by figsrc/build_quality_curves.py (data figsrc/data/ablation_std_curves.jsonl).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{quality_curve_psnr.pdf}

\caption[Our approximations cost little quality]{Our approximations cost little quality.\ {\normalfont
Test set quality metrics up to 30k iterations against training time over all \qaAllScenes{} scenes.}}
% CAPTION end
\Description{Two line charts against training time on an RTX 3070. Left, held-out PSNR: ours reaches 26.5 dB in 4.5 minutes; supervising every pixel at every step reaches the same PSNR after about 15 minutes; training on half-resolution images takes about the same time as ours but ends near 25.8 dB. Right, held-out SSIM: ours ends at 0.832 after 4.5 minutes; without Tile SSIM it ends slightly higher, at 0.833, after 5.2 minutes; with SH degree 3 and no cones it falls behind after about 2.5 minutes and ends at 0.829.}
\label{fig:quality_curve}
\end{figure}


==> diagrams/fig_stage_fwd.tex <==
% Forward rasterization variants: instructions per step on garden and stage time over 15 scenes. Plot generated by
% figsrc/build_stage_detail.py (fwd_plot; data figsrc/data/stage_detail_*, GS-CUDA-prof 7501b02, RTX 3070).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{stage_fwd.pdf}
\caption{Forward rasterization, step by step}
\Description{Two horizontal bar charts side by side for five forward-rasterization variants: instructions per step and stage time. Both fall from no subtile masks, to subtile masks, to added shared colour, to added hit lists, to both (ours).}
\label{fig:stage_fwd}
\end{figure}


==> diagrams/fig_stage_vram.tex <==
% Device memory on garden, ours and each within-stage alternative that changes it. Plot generated by
% figsrc/build_stage_vram.py (data figsrc/data/stage_detail_time.jsonl, GS-CUDA-prof 7501b02, RTX 3070).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{paper_figures/figures_out/stage_vram.pdf}
\caption{Device memory per alternative}
\Description{Horizontal stacked bars of device memory on garden for ours and eight alternatives, split into splat parameters, Adam moments, projected splats and gradients, keys and sort, per-pixel buffers and scratch.}
\label{fig:stage_vram}
\end{figure}


==> diagrams/fig_strided_sampling.tex <==
% Strided pixel sampling. 2026-11-20 (Nicholas): same style and scale as Fig. 6 (fig_mech_loss_pair_p1):
% thin black!14 pixel grid at 0.08 cm per pixel, rendered pixels shaded (black, fill opacity 0.18, over the grid), tile boundaries dgink 0.8 pt,
% no phase numbers. Each panel is the same 32x32-pixel screen region (2.56 cm): full resolution = four 16x16
% tiles, every pixel shaded; half resolution = one tile of 16x16 half-res pixels (2x2 screen px each), all
% shaded; strided = one 32x32 tile, one pixel of every 2x2 block shaded (phase 0 of this step).
% Previous version (numbered 1/4-scale cells): git history before this commit.
\begin{figure}[t]
\centering
\begin{tikzpicture}[dg]
  \tikzset{lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute},
           px/.style={black!14, line width=0.1pt}, tileb/.style={dgink, line width=0.8pt}}
  \def\p{0.08}    % one pixel (cm), as in Fig. 6
  \def\w{2.56}    % 32 pixels
  \def\gap{2.92}  % panel pitch: 3 panels across 8.4 cm
  % ---- (a) full resolution: every pixel, 16x16 tiles
  \begin{scope}[shift={(0,0)}]
    \draw[px, step=\p] (0,0) grid (\w,-\w);
    \fill[black, fill opacity=0.18] (0,0) rectangle (\w,-\w);
    \draw[tileb, step=16*\p] (0,0) grid (\w,-\w);
    \draw[tileb] (0,0) rectangle (\w,-\w);
  \end{scope}
  % ---- (b) half resolution: half-res pixels are 2x2 screen pixels; one tile of 16x16 half-res pixels
  \begin{scope}[shift={(\gap,0)}]
    \draw[px, step=2*\p] (0,0) grid (\w,-\w);
    \fill[black, fill opacity=0.18] (0,0) rectangle (\w,-\w);
    \draw[tileb] (0,0) rectangle (\w,-\w);
  \end{scope}
  % ---- (c) strided: one pixel of every 2x2 block rendered this step; one 32x32 tile
  \begin{scope}[shift={(2*\gap,0)}]
    \foreach \i in {0,...,15}{\foreach \j in {0,...,15}{%
      \fill[black, fill opacity=0.18] ({2*\i*\p},{-2*\j*\p}) rectangle ++(\p,-\p);}}
    \draw[px, step=\p] (0,0) grid (\w,-\w);
    \draw[tileb] (0,0) rectangle (\w,-\w);
  \end{scope}
  % ---- labels
  \foreach \i/\t/\s in {0/Full resolution \gm{(4 tiles)}/tile $16{\times}16$ pixels,
                        1/Half resolution/tile $16{\times}16$ half-res pixels,
                        2/Strided sampling/tile $32{\times}32$ pixels} {
    \node[lab, anchor=north west] at ({\i*\gap},-\w-0.12) {\textbf{\t}};
    \node[mut, anchor=north west] at ({\i*\gap},-\w-0.42) {\s};
  }
\end{tikzpicture}
% CAPTION (hand-edited, kept when the table is regenerated) begin
\caption[Strided pixel sampling]{Strided pixel sampling.\ {\normalfont
Cells are pixels and heavy lines are tile boundaries. Under half resolution a $16{\times}16$ tile covers the same screen area
   as a $32{\times}32$ tile under \nicefrac{1}{4} stride.}}
% old (2026-11-20, before the Fig. 6 style): Cells are pixels and heavy lines are tile boundaries, drawn at $1/4$ scale: a $4{\times}4$ block of cells is a $16{\times}16$ tile. Under half resolution ...
% old: \caption{\textbf{Strided pixel sampling.} Cells are pixels and heavy lines are tile boundaries, drawn at $1/4$ scale: a $4{\times}4$ block of cells is a $16{\times}16$ tile. Under half resolution a $16{\times}16$ tile covers the same screen area as a $32{\times}32$ tile under \nicefrac{1}{4} stride. Numbers mark the phase in which a pixel is rendered.}
% CAPTION end
\Description{Three pixel grids side by side, each the same 32 by 32 pixel area. Full resolution: every pixel shaded, heavy lines split the area into four 16 by 16 pixel tiles. Half resolution: the same area drawn as 16 by 16 larger shaded pixels, each 2 by 2 screen pixels, with one heavy outline as a single tile. Strided sampling: only one pixel of every 2 by 2 block is shaded, and one heavy outline around the area is a single 32 by 32 tile.}
\label{fig:sampling}
\end{figure}


==> diagrams/fig_visibility.tex <==
% Share of splats visible per view, stacked by scene. Plot generated by figsrc/build_visibility.py
% (data figsrc/data/visibility, from RESULTS_ARCHIVE/cone_runs/visibility_stats.py on the 15 bwd3147 v47 models).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{paper_figures/figures_out/visibility_hist.pdf}
\caption{\textbf{Most splats are not seen in a given view.} Share of splats with at least one tile, over every view of our 15 scenes, stacked by scene. A view sees 33\% on average; the projection backward and Adam skip the rest.}
\Description{A histogram of views by the percentage of splats visible, stacked by scene, peaking at 30 to 35 percent with a mean of 33 percent.}
\label{fig:visibility}
\end{figure}


==> diagrams/fig_visibility_muted.tex <==
% Share of splats visible per view, stacked by scene. Plot generated by figsrc/build_visibility_muted.py (muted copy, board variant 2026-11-14)
% (data figsrc/data/visibility, from RESULTS_ARCHIVE/cone_runs/visibility_stats.py on the 15 bwd3147 v47 models).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{paper_figures/figures_out/visibility_hist_muted.pdf}
\caption{\textbf{Most splats are not seen in a given view.} Share of splats with at least one tile, over every view of our 15 scenes, stacked by scene. A view sees 33\% on average; the projection backward and Adam skip the rest.}
\Description{A histogram of views by the percentage of splats visible, stacked by scene, peaking at 30 to 35 percent with a mean of 33 percent.}
\label{fig:visibility-muted}
\end{figure}


==> diagrams/fig_visibility_redblue.tex <==
% Share of splats visible per view, stacked by scene. Plot generated by figsrc/build_visibility_redblue.py (red/blue copy, board variant 2026-11-14)
% (data figsrc/data/visibility, from RESULTS_ARCHIVE/cone_runs/visibility_stats.py on the 15 bwd3147 v47 models).
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{paper_figures/figures_out/visibility_hist_redblue.pdf}
\caption{\textbf{Most splats are not seen in a given view.} Share of splats with at least one tile, over every view of our 15 scenes, stacked by scene. A view sees 33\% on average; the projection backward and Adam skip the rest.}
\Description{A histogram of views by the percentage of splats visible, stacked by scene, peaking at 30 to 35 percent with a mean of 33 percent.}
\label{fig:visibility-redblue}
\end{figure}


==> diagrams/spawn_panel.tex <==
% One-panel cone spawn (2026-11-14 board variant): fig_alt_spawn's two panels drawn as one picture, 4.1 cm wide.
% Same demo numbers as fig_alt_spawn.tex for the upper views: error views at 62/78/92/105/120 deg, mean axis
% 91.4 deg, k = 2.68 -> child cone half-angle arccos(1 - 1/k) = 51 deg (40..142 deg). Two extra grey views
% below (225/300 deg, ~0 counts) only widen the spread, so the rule still spawns. The light full disc is the
% original splat, seen from every direction; the shaded wedge is the child's opacity factor 1 - k (1 - cos phi)
% in 3-degree strips, as in the cone opacity panel. Use inside a tikzpicture[dg]; origin = top left.
  \tikzset{lab/.style={inner sep=0pt, text=dgink}, mut/.style={inner sep=0pt, text=dgmute},
           sray/.style={->, draw=dgink, line width=0.55pt, >={Latex[length=1.1mm, width=0.9mm]}},
           gray ray/.style={sray, draw=black!35, line width=0.45pt}}
  \node[lab, anchor=west] at (0,0) {\textbf{Add a cone splat at high-error views}};
  \begin{scope}[shift={(2.05,-1.95)}]
    \def\R{1.3}
    \fill[black!7] (0,0) circle (\R);
    \draw[dgmute, line width=0.3pt, densely dotted] (0,0) circle (\R);
    \foreach \i in {0,...,16} {
      \pgfmathsetmacro{\pa}{3*\i}
      \pgfmathsetmacro{\pb}{min(3*\i+3,50.6)}
      \pgfmathsetmacro{\g}{max(7,40*(1-2.68*(1-cos(3*\i+1.5))))}
      \fill[black!\g] (0,0) -- (91-\pb-0.4:\R) arc (91-\pb-0.4:91-\pa:\R) -- cycle;
      \fill[black!\g] (0,0) -- (91+\pa:\R) arc (91+\pa:91+\pb+0.4:\R) -- cycle;
    }
    \draw[dgink, line width=0.4pt] (0,0) -- (40:\R) (0,0) -- (142:\R);
    \draw[dgink, line width=0.4pt] (40:\R) arc (40:142:\R);
    \foreach \a/\v in {0/0, 25/0.3, 45/0.7, 135/0.5, 158/0.2, 180/0, 225/0, 300/0.1} {
      \draw[gray ray] (0,0) -- (\a:\R);
      \node[mut] at (\a:1.55) {\v};
    }
    \foreach \a/\v in {62/4, 78/15, 92/26, 105/18, 120/7} {
      \draw[sray] (0,0) -- (\a:\R);
      \node[lab] at (\a:1.52) {\v};
    }
    \fill[black!40, rotate=15] (-0.08,-0.03) ellipse (0.12 and 0.055);
    \fill[dgink, rotate=15] (0.06,0.04) ellipse (0.12 and 0.055);
  \end{scope}
  \node[mut, anchor=north west] at (0,-3.55) {number: high-error pixels the splat covers};
  \fill[dgink, rotate around={15:(0.17,-3.92)}] (0.17,-3.92) ellipse (0.12 and 0.055);
  \node[lab, anchor=north west] at (0.4,-3.83) {new: a copy, opacity 0.1, only in the cone};
  \fill[black!40, rotate around={15:(0.17,-4.2)}] (0.17,-4.2) ellipse (0.12 and 0.055);
  \node[mut, anchor=north west] at (0.4,-4.11) {original: kept, seen from every view};


==> diagrams/table_appearance.tex <==
% Cost of appearance (color + any view-dependent opacity term), per splat per view.
% Rows: color methods | opacity methods (each on top of its own color model) | ours.
% 2026-11-12 (Nicholas): dropped SH2, VDGS, N-DG (N-DG's cull is a separate conservative 3-sigma bound test, not
% a property of its opacity); read/written labelled as projection forward; last column = whether the view-dependent
% opacity can be exactly 0 and whether that is used to drop the splat before key emission.
% Sources (scratchpad appearance_methods.md survey + own code reads):
%   SH: Inria computeColorFromSH (preprocess, visible only, writes rgb).
%   Beta Splatting 431d575: SH0 + 2 spherical beta lobes, visible only.
%   Spec-Gaussian 0b40ce3 (released real-scene config): SH3 + 12-float ASG feature, 8 ASGs + MLP 31->32->3,
%       ~1.5k MAC, ~52 transcendentals, PyTorch, visible splats. Read = SH3 192 + 48.
%   Spherical Voronoi (MCMC backbone d813259): 8 sites x 7 floats = 56, CUDA preprocess, visible; 24 sqrt, 16 exp.
%   VoD-3DGS: no code; paper Eq. 10 sigmoid(gamma + w^T S w), SH degree 3 implied; assumed fused. Never 0.
%   UBS 1b502a4: opacity factor prod (1 - clamp(tanh y^2, 0, 1-eps))^beta, never 0; Sigma build 84/144 B +
%       conditioning 196/52 B, all splats.
%   ARF 57cca00: SH3; lobe exactly 0 for theta >= pi T but passed to unmodified gsplat, so the splat still gets keys.
%   Scaffold-GS 59c833b: opacity tanh(MLP) <= 0 -> child masked before the rasterizer (exact zero, used).
%       Per generated splat: read 304/10 ~ 30 B of anchor data, writes the generated Gaussian (56 B).
%   Ours: GS-CUDA cone f86b746.
% Traffic rule: parameters read + results written to global memory for a later kernel, in the projection forward
% (where appearance is evaluated), as released; PyTorch temporaries and shared network weights not counted; the
% rasterizer's own color read excluded for every row. Adam = floats x 12 B (parameter + two fp32 moments).
% 2026-11-19 (Nicholas): squeezed to one column. Beta Splatting dropped (not discussed in the text); Backward, Adam and
% Zero Opacity columns cut (Adam = Floats x 12 B, said in the caption); Read/Write/Work are the projection forward,
% before rasterization (said in the caption). Previous full-width table kept below as comments.
% 2026-11-19 (Nicholas): color-model suffixes (", SH3", ", RGB") dropped from the opacity rows -- the color model is
% now the first item of Work; Work shortened (MAD = multiply-add; clamps dropped; UBS "all splats" -> footnote u).
\begin{table}[t]
    \centering
    % CAPTION (hand-edited, kept when the table is regenerated) begin
    \caption[View-dependent color and opacity models]{View-dependent color and opacity models.\ {\normalfont Read, Write in Bytes, Work: computation needed. MAD: multiply-add.
   $^{s}$Per generated splat: an anchor of
   76 floats yields 10.}}
    % old: \caption{\textbf{What appearance costs}, per splat per view.}
    % CAPTION end
    \footnotesize
    \renewcommand{\arraystretch}{1.1}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l r r r >{\raggedright\arraybackslash}p{3.3cm}@{}}
    \toprule
     & Floats & Read & Write & Work \\
    \midrule
    SH0                                   & 3  & 12\,B  & 12\,B & 3 MADs \\
    SH3 (3DGS~\cite{kerbl20233dgs})       & 48 & 192\,B & 12\,B & 16 basis values, 48 MADs \\
    Spec-Gaussian~\cite{yang2024specgaussian} & 60 & 240\,B & 12\,B & SH3, 8 ASGs, MLP (1.5k MACs) \\
    Sph.\ Voronoi~\cite{disario2025sphericalvoronoi} & 56 & 224\,B & 12\,B & 8 sites, 24 sqrt, 16 exp \\
    \midrule
    % 2026-11-19 (Nicholas) cut: VoD-3DGS~\cite{nowak2025vod3dgs}$^{p}$ & 54 & 216\,B & 12\,B & SH3, quadratic, sigmoid \
    UBS~\cite{liu2026ubs}           & 24 & 280\,B & 196\,B & RGB, $6{\times}6\,\Sigma$, 3 tanh, 3 pow \\
    ARF~\cite{yang2026arf}          & 53 & 212\,B & 16\,B & SH3, dot, acos, cos, pow \\
    Scaffold-GS~\cite{lu2024scaffoldgs}$^{s}$ & 7.6 & 30\,B & 56\,B & 3 MLPs (690 MACs) \\
    \midrule
    {\textbf\name} (RGB)                            & 3  & 0\,B   & 0\,B  & None \\
    {\textbf\name}  (RGB $+$ cone)                   & 7  & 16\,B  & 0\,B  & normalize, dot, MAD \\
    \bottomrule
    \end{tabular*}
    \label{tab:appearance}
\end{table}
%
% ---- previous full-width version (before 2026-11-19)
% \begin{table*}[t]
%     \centering
%     \caption{\textbf{What appearance costs}, per splat per view. Top: view-dependent color; middle: view-dependent opacity on the named color model. Floats: per-splat parameters. Forward and backward: global-memory bytes for appearance outside the rasterizer. Adam: parameters plus two fp32 moments, ours included. Zero opacity: whether opacity can be exactly zero, and whether such a splat is dropped before keys. $^{p}$From the paper; no public code. $^{a}$Lobe on about 10\% of splats; the row is per such splat. $^{s}$Per generated splat: an anchor of 76 floats yields 10.} % ya: caption should be above the table
%     \footnotesize
%     \renewcommand{\arraystretch}{1.12}
%     \setlength{\tabcolsep}{3.2pt}
%     \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l r r r >{\raggedright}p{5.6cm} >{\raggedright}p{3.0cm} r >{\raggedright\arraybackslash}p{2.4cm}@{}}
%     \toprule
%      & & \multicolumn{3}{c}{Forward, Before Rasterization} & \multicolumn{1}{c}{Backward} & & \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-6}
%      & Floats & Read & Write & Work & Work & Adam & Zero Opacity \\
%     \midrule
%     SH degree 0                 & 3  & 12\,B  & 12\,B & 3 multiply-adds, clamp & 3 gradients, clamp mask & 36\,B & --- \\
%     SH degree 3 (3DGS~\cite{kerbl20233dgs}) & 48 & 192\,B & 12\,B & 16 basis values, 48 multiply-adds, clamp & 48 gradients, $+\,\partial c/\partial d$ & 576\,B & --- \\
%     Beta Splatting~\cite{liu2025betasplatting}, 2 lobes & 15 & 60\,B  & 12\,B & SH0, then per lobe: 2 sincos, dot, pow, exp & 15 gradients, $+\,\partial c/\partial d$ & 180\,B & --- \\
%     Spec-Gaussian~\cite{yang2024specgaussian} & 60 & 240\,B & 12\,B & SH3, 8 anisotropic SGs, MLP ($\approx$1.5k MACs, $\approx$50 exp) & 60 gradients, $+$ MLP & 720\,B & --- \\
%     Spherical Voronoi~\cite{disario2025sphericalvoronoi}, 8 sites & 56 & 224\,B & 12\,B & 8 distances, softmax: 24 sqrt, 16 exp & 56 gradients, $+\,\partial c/\partial d$ & 672\,B & --- \\
%     \midrule
%     VoD-3DGS~\cite{nowak2025vod3dgs}$^{p}$, SH3 & 54 & 216\,B & 12\,B & SH3, then quadratic form, sigmoid & 54 gradients, $+\,\partial/\partial d$ & 648\,B & Never \\
%     UBS~\cite{liu2026ubs}, RGB & 24 & 280\,B & 196\,B & build, condition $6{\times}6\,\Sigma$, 3 tanh, 3 pow; all splats & 21 gradients, $+$ chain to mean & 288\,B & Never \\
%     ARF~\cite{yang2026arf}$^{a}$, SH3 & 53 & 212\,B & 16\,B & SH3, then dot, acos, cos, pow & 53 gradients, $+\,\partial/\partial d$ & 636\,B & Exact, unused \\
%     Scaffold-GS~\cite{lu2024scaffoldgs}$^{s}$, MLP & 7.6 & 30\,B & 56\,B & 3 MLPs give color, opacity, shape ($\approx$690 MACs) & MLP and anchor gradients & 91\,B & Exact, splat dropped \\
%     \midrule
%     Ours (direct color)         & 3  & 0\,B   & 0\,B  & None & 3 gradients, copied & 36\,B & --- \\
%     Ours (direct $+$ cone)       & 7  & 16\,B  & 0\,B  & normalize $w$, dot, multiply-add, clamp & 4 gradients, $+\,\partial\alpha'/\partial x$ & 84\,B & Exact, splat dropped \\
%     \bottomrule
%     \end{tabular*}
%     \label{tab:appearance}
% \end{table*}


==> diagrams/table_bwd_ablation.tex <==
% generated by figsrc/build_bwd_ablation.py from figsrc/data/bwd_ablation.jsonl
\begin{table}[t]
    \centering
    \caption{\textbf{Rasterize backward.} Kernel time, geometric mean over 15 scenes at full resolution (RTX 3070). gsplat~\cite{ye2024gsplat} and Taming~\cite{mallick2024taming} are ports into our pipeline. Speedup is against gsplat.}
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l l r r@{}}
        \toprule
        Traversal & Change & Time (ms) & Speedup \\
        \midrule
        Per pixel & gsplat~\cite{ye2024gsplat} & 9.84 & 1.00$\times$ \\
        Per splat & Taming~\cite{mallick2024taming} & 7.80 & 1.27$\times$ \\
        \midrule
        Per chunk & standard pair arithmetic & 3.55 & 2.78$\times$ \\
         & + arithmetic optimizations & 3.14 & 3.16$\times$ \\
         & + skip unreached chunks & 2.97 & 3.33$\times$ \\
         & + wait per chunk (ours) & 2.82 & 3.51$\times$ \\
        \bottomrule
    \end{tabular*}
    \label{tab:bwd-ablation}
\end{table}


==> diagrams/table_bwd_occupancy.tex <==
% generated by figsrc/build_bwd_occupancy.py from figsrc/data/bwd_occupancy_ncu.json, bwd_ablation.jsonl, bwd_vksplat.jsonl
\begin{table}[t]\centering\scriptsize
\setlength{\tabcolsep}{0pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rrr rl rr r@{}}
\toprule
 & & & Shared & \multicolumn{2}{c}{Blocks per SM} & \multicolumn{2}{c}{Occupancy} & Speedup \\
Kernel & Threads & Regs & (B) & & limited by & theor. & achieved & vs gsplat \\
\midrule
gsplat~\cite{ye2024gsplat} & 256 & 40 & 10{,}240 & 6 & regs+threads & 100\% & 94\% & 1.00$\times$ \\
Taming-3DGS~\cite{mallick2024taming} & 32 & 61 & 772 & 16 & 16 cap & 33\% & 33\% & 1.27$\times$ \\
VkSplat~\cite{vksplat} & 128 & 56 & 9{,}216 & 9 & regs & 75\% & 75\% & 1.72$\times$ \\
\midrule
A & 128 & 55 & 9{,}220 & 9 & regs+shared & 75\% & 75\% & 2.11$\times$ \\
B & 128 & 47 & 8{,}208 & 10 & regs+shared & 83\% & 83\% & 2.85$\times$ \\
C & 128 & 48 & 8{,}816 & 10 & regs+shared & 83\% & 83\% & 3.29$\times$ \\
D & 128 & 48 & 8{,}816 & 10 & regs+shared & 83\% & 82\% & 3.35$\times$ \\
E & 128 & 48 & 9{,}216 & 10 & regs+shared & 83\% & 83\% & 3.47$\times$ \\
\bottomrule
\end{tabular*}
\caption{\textbf{Rasterize backward: registers, shared memory and occupancy.}}
\label{tab:bwd-occupancy}
\end{table}


==> diagrams/table_projadam_ablation.tex <==
% generated by figsrc/build_projadam_ablation.py from figsrc/data/projadam_ablation.jsonl + projadam_ncu.json
\begin{table*}[t]\centering\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l | c c c | r r r | r r r | r r r@{}}
\toprule
 & fused & sparse & compact & \multicolumn{3}{c|}{visible splat} & \multicolumn{3}{c|}{unseen splat} & \multicolumn{3}{c}{stage time} \\
 & kernel & Adam & moments & read (B) & written (B) & instr. & read (B) & written (B) & instr. & ms & Speedup & Step \\
\midrule
gsplat~\cite{ye2024gsplat}$^{a}$ &  & \checkmark &  & 1829 & 2229 & 10.8k & 525 & 1178 & 6.8k & 10.87 & 1.00$\times$ &  \\
VkSplat~\cite{vksplat}$^{b}$ & \checkmark &  &  & 748 & 744 & 2.2k & 712 & 744 & 1.1k & 5.67 & 1.92$\times$ &  \\
LichtFeld~\cite{lichtfeld}$^{c}$ & \checkmark &  & \checkmark & 737 & 560 & 13.0k & 535 & 449 & 11.9k & 8.78 & 1.24$\times$ &  \\
\midrule
\multicolumn{13}{@{}l}{\textit{Combining ideas}} \\
1.\ + fused kernel & \checkmark & \checkmark &  & 748 & 744 & 2.2k & 4 & 36 & 12 & 2.41 & 4.51$\times$ & 4.51$\times$ \\
2.\ + bf16 moments & \checkmark & \checkmark & \checkmark & 512 & 508 & 3.5k & 4 & 36 & 12 & 1.76 & 6.19$\times$ & 1.37$\times$ \\
3.\ + RGB and cone & \checkmark & \checkmark & \checkmark & 184 & 180 & 1.3k & 4 & 36 & 12 & 0.67 & 16.25$\times$ & 2.62$\times$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Projection backward and Adam.} Fused: the backward and Adam share a thread, so no gradient buffer. Sparse: splats with no tile in the view are skipped. Compact moments: 16 bits or fewer. Bytes are DRAM per visible or unseen splat, from the code and checked with Nsight Compute; instructions per splat on garden. Time: whole stage, mean over 15 scenes (RTX 3070). All rows run in our pipeline at SH degree 3 except RGB and cone; gsplat, VkSplat and LichtFeld are timed in their own code during training, scaled to our splat counts. Speedup is against gsplat, Step against the row above. $^{a}$With its sparse Adam on. $^{b}$Bytes and instr.\ of our CUDA rebuild of its Vulkan kernel. $^{c}$Its kernel compiled in our bench.}
\label{tab:projadam-ablation}
\end{table*}


==> diagrams/table_projadam_ablation_compact.tex <==
% generated by figsrc/build_projadam_ablation.py (table_compact) from figsrc/data/projadam_ablation.jsonl + projadam_ncu.json
\begin{table}[t]
    \centering
    % CAPTION (hand-edited, kept when the table is regenerated) begin
    \caption[Backward projection and Adam stage ablation]{Backward projection and Adam stage ablation.\ {\normalfont
    Read/write (Bytes): DRAM traffic per visible/unseen splat}}
    % old: \caption{\textbf{Projection backward and Adam stage ablation.} Read/write (Bytes): DRAM bytes per visible/unseen splat; Instr.: instructions per splat on garden. Time (ms): whole stage, mean over 15 scenes on RTX~3070; the first three rows are timed in their own code during training, capped at our splat counts. All rows run at SH degree 3 except the last. $^{a}$With its sparse Adam on. $^{b}$Bytes and instr.\ of our CUDA rebuild of its Vulkan kernel. $^{c}$Its kernel compiled in our bench.}
    % CAPTION end
    \footnotesize
    \setlength{\tabcolsep}{0.7pt}
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l ccc | ccc | ccc | c@{}}
        \toprule
         & Fused & Sparse & Comp. & \multicolumn{3}{c|}{Visible Splat} & \multicolumn{3}{c|}{Unseen Splat} & Time \\
         & Kernel & Adam & Mom. & Read & Write & Instr. & Read & Write & Instr. & (Speedup) \\
        \midrule
        gsplat~\cite{ye2024gsplat}$^{a}$ &  & \checkmark &  & 1.8k & 2.2k & 11k & 0.5k & 1.1k & 6.8k & 10.9 (1.00$\times$) \\
        VkSplat~\cite{vksplat} & \checkmark &  &  & 0.7k & 0.7k & 2.2k & 0.7k & 0.7k & 1.1k & 5.67 (1.92$\times$) \\
        LichtFeld~\cite{lichtfeld} & \checkmark &  & \checkmark & 0.7k & 0.5k & 13k & 0.5k & 0.4k & 12k & 8.78 (1.24$\times$) \\
        \midrule
        + fused kernel & \checkmark & \checkmark &  & 0.7k & 0.7k & 2.2k & 4 & 36 & 12 & 2.41 (4.51$\times$) \\
        + bf16 moments & \checkmark & \checkmark & \checkmark & 0.5k & 0.5k & 3.5k & 4 & 36 & 12 & 1.76 (6.19$\times$) \\
        + RGB and cone & \checkmark & \checkmark & \checkmark & 0.2k & 0.2k & 1.3k & 4 & 36 & 12 & 0.67 (16.2$\times$) \\
        \bottomrule
    \end{tabular*}
    \label{tab:projadam-ablation}
\end{table}


==> sec/1_intro_old.tex <==
% 1_intro_alt.tex -- ALTERNATIVE opening for the introduction.
\section{Introduction}
\label{sec:intro}
% \gm{Title: "Usable scene" sounds good, but we need to define what "usable" means quantitatively (e.g., time-to-target quality). Otherwise consider "Full-Resolution Gaussian Splatting in Minutes on Consumer GPUs".}
% \gm{Maybe start a little bit for further context to highlight how popular 3DGS has become for capture and representing 3D scenes... but there is a gap on using it with/on common place devices.}

% Text from Nicholas's notes docx (2026-11-13), prepended to the existing intro.
As of late, 3D Gaussian Splatting~\cite{kerbl20233dgs} has established itself as the premier method for capturing 3D scenes for use in novel view synthesis or scene analysis/editing, showcasing efficient training and rendering performance and quality.
With performance, many techniques improve training time, model size, memory use and rendering speed. But these optimizations are often localized to one or a few stages of the training pipeline. Surveying the field \ya{(\cref{sec:related})}, the number of options and training configurations can be overwhelming, and popular implementations end up as an \gm{amalgam} of techniques \gm{originally separately proposed}.
There is a gap in diagnosis and unified breakdown of all stages of training, and subsequently a training system that considers the whole pipeline together.

Tractable for radiance field training at inception, works pushed hard on training
speed, bringing scene fitting down from hours to a few minutes~\cite{mallick2024taming,fastgs,chen2025dashgaussian,fang2024minisplatting2,dhiman2024turbogs}. But once training deviates from the capped training resolution and research-grade hardware configurations, it quickly becomes impractical.

Firstly, standard Mip-NeRF~360 protocol downsamples captures to
1.0--1.6 megapixels~\cite{barron2022mipnerf360}, and the 3DGS reference
implementation rescales inputs wider than 1600 pixels by
default~\cite{kerbl20233dgs}, so nearly all reported results supervise at a
fraction of the resolution actually captured. 
When scaling up training resolution, the loss, backward rasterization, key emission and sorting stages of a training step all scale with the number of supervised pixels and become several times more expensive. Resolution is consequently treated as the first thing to give up, even when its cost as essentially an approximation has not been measured.
%
A second obstacle is the hardware assumed. Accelerated variants report great improvement with standard research-grade GPUs, but such devices are out of reach for the general public or even hobbyists. Consumer-level GPUs often have limits on VRAM and bandwidth which cause certain stages in training to be disproportionately slower. Per-stage timings, as a proportion of total training time, shift. 


Our goal is to keep as few assumptions as possible and prioritize overall performance that scales with 1) splats, 2) resolution, 3) limited compute capability.
We rebuild every stage of training, question every parameter and operation, to eliminate all unnecessary assumptions that hurt performance.

% Contribution 2026-11-16 at Nicholas's request: bullets dropped, per-stage breakdown no longer claimed;
% the full-system sentence is the old second bullet (Claude-condensed, NOT YET VETTED). Earlier lists in git history.
Our contribution is a full training system that reworks every stage of the step for full-resolution training on consumer GPUs: a leaner splat with flat RGB color and a directional cone opacity, projection and key generation fused into one pass, strided pixel sampling, a single-kernel tile-based SSIM loss, a warp-per-splat backward rasterization, and projection backward fused with a sparse Adam step over bf16 moments (\cref{sec:appearance,sec:projkeys,sec:fwd,sec:loss,sec:bwd,sec:adam}) \gmc{Maybe refer to Figure 2 here}. We evaluate \gm{our proposed method} against prior fast 3DGS trainers at full resolution on consumer GPUs (\cref{sec:results}).

\yac{I think we should say more in this section. This is the most important section while I think currently we haven't speak out loudly enough about our brilliant contributions. I will try to polish it.} \gmc{I agree that the work could be put into a more convincing perspective. %WT is also very good for that. -there is so many people using 3DGS these days, that you may have an impact on global energy consumption ! 
}


\papfig{Per-stage timings}{tables/table_stage_shift}

==> sec/archive/3_method_old.tex <==
\section{Method}
\label{sec:method}
% ANAND: Let us separate Method, main Results, and Ablation more clearly. % Sec. 4 should describe WHAT we do and WHY the design is reasonable, % without embedding quantitative evaluation. % Proposed order: Sec. 4 Method -> Sec. 5 Results -> Sec. 6 Ablation/Analysis.
% ANAND: ORGANIZATION FOR SEC. 4.4

% \gm{Is it possible to have a very first section that shows the time/computation budget of each step, so that the reader is convienced (as you are ;) that you focus on the important steps ? --Maybe it would be good to start also the 3DGS pipeline to recall important steps, quantify the time and ressurces taken by each, and locate your work and contribution, showing that your choices on the stages your consider are cohenrent.
% }
% ANAND: Yes, I think this would help. Add a short subsection at the
% beginning of Method showing the standard 3DGS training pipeline and
% where the computation goes at full resolution (use RTX 3070 as the
% representative consumer GPU).
%
% A simple pipeline/timing figure is enough -- e.g.,
% projection/key generation -> sort -> rasterization forward ->
% loss/SSIM -> rasterization backward -> optimizer/densification.
%
% Highlight the stages targeted by our method and briefly state why:
% backward rasterization and SSIM are major bottlenecks, while key
% generation/sorting also grow with resolution. Pixel sampling is then
% introduced as a complementary way to reduce work while retaining
% native-resolution supervision.
%
% We already have the stage timing data in the Appendix (Fig. 9/Table 8),
% so simplify/reuse this rather than adding another experiment.

\subsection{Standard 3DGS Training Pipeline}
\label{sec:pipeline}
\input{sec/archive/table_pipeline_profile}

The stages of a step in 3DGS training are projection, key generation, sort, rasterization, loss, rasterization backward, projection backward, optimizer and densification. The costs are not spread
evenly across stages (\cref{tab:pipeline-profile}). We briefly describe the stages our approach touches.

After projecting 3D Gaussians to 2D splats, the keys stage produces Gaussian-Tile pairs each representing an intersection of a Gaussian and a tile. Scaling resolution increases the number of tiles, which means there are more pairs. It is a relatively minor stage and we make a small optimization in (\cref{sec:keys-stage}).

The loss stage compares the image rendered by the 3DGS model against the ground truth image, taking L1 and SSIM losses. Scaling resolution, SSIM loss becomes expensive, we address this in (\cref{sec:tile-ssim}).

The backward rasterization stage takes the image loss and computes gradients for the 2D projected splats. It is the major compute bottleneck of the pipeline. We make optimizations to this stage in (\cref{sec:backward}).

We adapt a key contribution of TurboGS in Forward rasterization (\cref{sec:sampling}), and adapt densification from Fast-GS. We also use Sparse Adam, details in (\cref{sec:details}). Our codebase is built on top of VkSplat's released work~\cite{vksplat}.

\input{sec/archive/KEYS_SECTION}
\input{sec/archive/SSIM_SECTION}
\input{sec/archive/BACKWARD_SECTION}
\input{sec/archive/SAMPLING_SHORT}
\input{sec/archive/DETAILS_SECTION}


==> sec/archive/BACKWARD_SECTION.tex <==
% ===================================================================
% Backward implementation -- paper subsection
% Requires: \usepackage{amsmath, amssymb, booktabs}

\subsection{Rasterization Backward: Front-to-Back}
\label{sec:backward}

% ANAND: ORGANIZATION FOR SEC. 4.3
%
% Keep here:
% - what gradient buffers are required (Table 4);
% - why the conventional backward traversal reconstructs transmittance;
% - the proposed front-to-back traversal and its computational rationale;
% - conceptual explanation of checkpointing.
%
% Move quantitative comparisons of traversal/checkpoint variants
% (Fig. 6 and Table 5) to Sec. 6.3.
%
% Method should explain the implementation choice; Sec. 6.3 should
% demonstrate its timing/VRAM consequences.
%
% ANAND: KEEP Table 4 here.
% This table describes the data/gradient buffers required by the backward
% pass and helps the reader understand the implementation. It is descriptive
% of the method rather than an ablation result.
%
% \gm{a little dry on jumping into the pipeline...}
Differentiating alpha blending requires, for every contributing
(pixel, splat) pair, two quantities from the forward pass: the
transmittance $T$ prevailing when that splat was blended, and the colour
accumulated by the splats behind it. Neither is stored, so both must be
reconstructed.

Reference implementations reconstruct them by walking the sorted list
back-to-front and undoing each blend by division,
%
\begin{equation}
  T_{i-1} \;=\; \frac{T_i}{1-\alpha_i},
  \qquad
  \mathbf{c}_{i-1} \;=\; \mathbf{c}_i - \alpha_i \mathbf{rgb}_i\, T_{i-1},
  \label{eq:undo}
\end{equation}
%
seeded from the stored $T_{\text{final}}$.

We observe the reverse walk is not necessary. Because the forward pass
already stores the final accumulated colour $A_{\text{final}}$ and final
transmittance $T_{\text{final}}$, the state can be seeded exactly at the
front of the list ($T = 1$, $ar = -A_{\text{final}}$) and the same
gradients recovered walking front-to-back --- the suffix colour the
gradient needs is $A_{\text{final}} - A_{\text{prefix}}$.

Because of the implementation details of walking from front-to-back, we have less per-pixel state to carry, more accurate transmittance, explicit closed-form gradients in
place of autodiff-generated adjoint recurrences, and 4 fewer registers required per thread.

Checkpoints (as in Taming-3DGS) store per-pixel state every $N$ splats,
letting segments at different depths be processed independently and raising
the parallelism available to the device. The benefit depends on how
work-starved the device is: against a checkpoint-free kernel it is
$1.55\times$ when tiles are few and deep, ${\sim}1.0\times$ when tiles are
many and shallow, and ${\sim}1.07\times$ at full resolution on a 3M-splat
scene. It comes with additional cost in the forward render stage for
checkpoint writes and additional VRAM usage for resident tables. As we are
targeting consumer devices, we expect the backward render pass to already
saturate the GPU with work, hence we elect not to use checkpoints.


==> sec/archive/DETAILS_SECTION.tex <==
% Other details -- last subsection of Method.
%
% NOTE: sec/OTHERS_SECTION.tex also carries a "\subsection{Other details}".
% It is dead (nothing \inputs it) and its body is an older copy of the
% sampling text, not this. Do not confuse the two; this is the live one.
%
% Drafted from the source, not from prose:
%   FASTGS.md            -- what the port changes vs the reference CUDA repo,
%                           and why the stats accumulation is strided at all
%   vksplat/train_checker.py  -- why the stride is 5 rather than the default 4
%   vksplat/ablation_arm{,2}.py -- the fleet runs that produced the F0-F5 data
%                           set fastgs_stats_every = 5, so 5 is the paper's value
%   slang/config.slang   -- ADAM_CULL_INVISIBLE says in as many words that
%                           upstream SparseGaussianAdam does NOT compensate

\subsection{Other Details}
\label{sec:details}
Densification follows FastGS~\cite{fastgs}, with a minor adjustment in implementation. In FastGS, a score is computed at each densification interval by sampling training cameras and rendering, incurring a batch of extra forward passes per event on top of training. We instead accumulate the same statistic from the renders that training already produces, so densification incurs no additional renders.

When a training step ends, the composited image, the per-pixel contributor counts and the ground truth are all still resident, making it an ideal time to take the metric with an additional pixel pass.
We do so every 5 training steps, and execute the densification with the accumulated metrics every 100 steps (as per FastGS).

The optimizer takes a sparse Adam step, updating only the Gaussians that were
visible on the step, as recent accelerated trainers do~\cite{mallick2024taming,fastgs}.

==> sec/archive/KEYS_SECTION.tex <==
% Keys stage -- fused emission. Method section + figure.
% Preamble requirements:
%   \usepackage{amsmath}
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta, positioning, fit, calc}

\subsection{Keys Stage: Fused}
\label{sec:keys-stage}

In the original keys stage, producing the Gaussian--tile pairs list involves
twice enumerating the Gaussian--tile intersections. The first is performed by projection itself, 
which computes and discards each splat's exact ellipse--tile spans to report only its total number of intersections. A prefix sum over these counts sizes the sort buffer and assigns each splat a write
offset. A second kernel re-reads every splat's projected state from memory,
redoes the enumeration, and writes the Gaussian--tile pairs at the assigned
offsets.

In the original, the sort buffer fits the number of pairs perfectly, and there is an ordering for splats for where to write their pairs. But these are not properties required or helpful for training, since the ordering would be disrupted by the sort stage following it anyway.

We condense the two passes into one. The sort buffer
is pre-allocated at an ample capacity derived from peak historical iterations. Then projection proceeds, and a splat's ellipse--tile spans are calculated. 
Within a workgroup, each wave prefix-sums its lanes' pair counts, then does a single atomic addition on a global cursor to reserve a contiguous range in the pre-allocated sort buffer.
Finally, each lane derives its own write offset in the sort buffer from the prefix sum and workgroup's offset. 



==> sec/archive/SAMPLING_SHORT.tex <==
% ===================================================================
% Systematic sampling of pixels -- SHORT version (author's prose kept)
% Requires: \usepackage{amsmath, tikz}
% Colours (add to preamble if undefined):
%   \definecolor{wacvblue}{HTML}{2B6CB0}
%   \definecolor{colrtwo}{HTML}{B7791F}
%   \definecolor{colck}{HTML}{2F855A}
%   \definecolor{colckf}{HTML}{6B46C1}
% ===================================================================

\subsection{Rasterization Forward: Strided Pixel Sampling}
\label{sec:sampling}
% \gm{it is not very clear to me on how this section is linked to the tile SIMM Section !? Maybe you could clarify ?}
TurboGS first introduces 'Dilated Rendering', where a systematically strided subset of full-resolution images is used to train instead of using downsampled images. We adopt this idea and make some implementation changes, but our implementation does not quite have the dilation element and so we will refer to it as 'Strided Pixel Sampling'. 

We hypothesise that as training resolution rises, neighbouring pixels may
contribute increasingly similar gradients to the Gaussians they cover, so a
strided subset of a full-resolution image may supervise competitively at a lower cost. 

We evaluate two variants. The first, \emph{\nicefrac{1}{2} stride}, splits each
training image into two half-density images in a checkerboard-like pattern. The
second, \emph{\nicefrac{1}{4} stride}, splits it into
four, on a $2{\times}2$ grid, so that each step supervises $WH/4$ pixels---the
same per-iteration pixel budget as half-resolution (which has quarter number of pixels), but with four phases covering the full-resolution image over four steps.

We highlight the differences in our implementation with TurboGS's. Firstly, instead of reducing the number of threads per workgroup, we increase the tile size so that the number of pixels rendered per tile per iteration is unchanged. A tile (which is usually $16{\times}16$ in both full and half-resolution training) covers a $32{\times}16$ screen rectangle under \nicefrac{1}{2} stride and $32{\times}32$ under \nicefrac{1}{4} stride. The \nicefrac{1}{4} stride scheme and half resolution therefore render the same number of pixels per tile over the same screen area
(Fig.~\ref{fig:sampling}). Not having a reduced thread count has a positive impact on performance, and also reduces the number of tiles.

Secondly, we do this for the entire training, with no progressive resolution schedule. Each training image is first split into two/four separate images prior to training and stays that way throughout. This is to avoid loading the full image at each step. Total memory usage (for holding training images) stays unchanged.

Lastly, Turbo-GS applies a lattice-matched blur for compensation, which we do not. 

% Because the stride is regular, the implementation stays cheap: tile lists, keys and sort stages are
% phase-independent and hence require no change. Per-pixel buffers can be sized
% down to $WH/2$ and $WH/4$ for the two- and four-phase schemes respectively, and
% the split training images are compacted the same way. 

% \gm{For the whole Section \ref{sec:method} you could give for each subsection a qualitative hint on how your method improves, refereing to the corresponding quantitative results in the next (Results) section.  }

\begin{figure}[t]
  \centering
  \newcommand{\cellsc}{0.38}
  % \cbpanel{phase expr in \sx,\sy}{colour}{tile width}{tile height}{digits?}
  %   \sx : screen x, \sy : screen y measured DOWNWARDS from the top, so the
  %         phase expressions are verbatim those in the implementation.
  \newcommand{\cbpanel}[5]{%
    \begin{tikzpicture}[scale=\cellsc, line join=round,
                        baseline=(current bounding box.center)]
      \foreach \sx in {0,...,7}{%
        \foreach \sy in {0,...,7}{%
          \pgfmathtruncatemacro{\ph}{#1}%
          \pgfmathtruncatemacro{\yy}{7-\sy}%
          \ifnum\ph=0\relax
            \fill[#2] (\sx,\yy) rectangle ++(1,1);
            \ifnum#5=1\relax
              \node[font=\tiny, text=white, inner sep=0pt]
                at ({\sx+0.5},{\yy+0.5}) {0};
            \fi
          \else
            \fill[#2!12] (\sx,\yy) rectangle ++(1,1);
            \ifnum#5=1\relax
              \node[font=\tiny, text=#2!70!black, inner sep=0pt]
                at ({\sx+0.5},{\yy+0.5}) {\ph};
            \fi
          \fi
        }%
      }%
      \draw[white, line width=0.4pt] (0,0) grid (8,8);
      \draw[black!80, line width=1.4pt] (0,0) grid[xstep=#3, ystep=#4] (8,8);
      \draw[black!80, line width=1.4pt] (0,0) rectangle (8,8);
    \end{tikzpicture}%
  }
  % -r 2: one sample (dot) serves the 2x2 block of full-resolution pixels
  % drawn dashed beneath it -- the block IS one prefiltered GT pixel.
  \newcommand{\rtwopanel}{%
    \begin{tikzpicture}[scale=\cellsc, line join=round,
                        baseline=(current bounding box.center)]
      \foreach \i in {0,2,4,6}{\foreach \j in {0,2,4,6}{%
        \fill[colrtwo] (\i,\j) rectangle ++(2,2);
        \draw[white!65!colrtwo, line width=0.35pt,
              dash pattern=on 1.1pt off 1.1pt]
          ({\i+1},{\j}) -- ({\i+1},{\j+2})
          ({\i},{\j+1}) -- ({\i+2},{\j+1});
        \fill[white] ({\i+1},{\j+1}) circle (0.26);
      }}%
      \draw[white, line width=1.0pt] (0,0) grid[step=2] (8,8);
      \draw[black!80, line width=1.4pt] (0,0) rectangle (8,8);
    \end{tikzpicture}%
  }
  \begin{tabular}{@{}c@{\hskip 10pt}c@{}}
    \cbpanel{0}{wacvblue}{4}{4}{0} & \rtwopanel \\[2pt]
    % One line each: dropping the per-step percentage (the caption states it,
    % and the shading shows it) and shortening the names to "stride" brings
    % every label under the panel width, so the two-line \shortstack is gone.
    {\scriptsize (a) full-res\,\textbar\,tile $16{\times}16$} &
    {\scriptsize (b) half-res\,\textbar\,tile $16{\times}16$} \\[7pt]
    \cbpanel{mod(\sx+\sy,2)}{colck}{8}{4}{1} &
    \cbpanel{mod(\sx,2)+2*mod(\sy,2)}{colckf}{8}{8}{1} \\[2pt]
    {\scriptsize (c) \nicefrac{1}{2} stride\,\textbar\,tile $32{\times}16$} &
    {\scriptsize (d) \nicefrac{1}{4} stride\,\textbar\,tile $32{\times}32$} \\
  \end{tabular}

  \caption{%
    \textbf{Strided pixel sampling illustration}. Cells are pixels,
    heavy lines are tile boundaries drawn at $1/4$ scale for visualising relative tile sizes. For example in a), the tile is $4*4$ on figure, representing $16*16$ in implementation.
    Every tile holds exactly $256$ shaded cells ($16$ in diagram). In (b) the
    tile is a $16*16$ over a half-resolution image, covering the same area as 1/4 strided $32*32$ tile over full-resolution image.}
  \label{fig:sampling}
\end{figure}

==> sec/archive/SSIM_SECTION.tex <==

\subsection{Loss Stage: Tile SSIM}
\label{sec:tile-ssim}

The $\mathcal{L}_1$ and SSIM terms of the training loss are evaluated over every
pixel of the rendered image, so cost scales with resolution independently
of scene complexity. As resolution grows, the loss stage occupies an
increasing fraction of each training step. 
% The three shares below do not share a source. Read this before editing them:
%   * FULL resolution is reproducible from figsrc/data/active.json. F5 is the
%     baseline arm and runs the reference SSIM; on garden its loss stage is
%     16.0 percent of the step on the 3090, 17.5 on the 3070 and 12.3 on the
%     3060, and is second to backward rasterization on all three. 16 is the
%     3090 figure. The share is card-dependent, so do not restate it as if it
%     were a single number.
%   * QUARTER and HALF resolution are not reproducible from anything in this
%     repo. active.json has no r4 runs at all, and its r2 runs use our tile
%     SSIM rather than the reference. Both were measured off-repo, and their
%     only appearance in the paper was loss_share.pdf, which was removed on
%     2026-08-29 -- so as it stands these two numbers have no evidence in the
%     paper. Either the r4/r2 reference-SSIM timings land in figsrc/data/ and
%     this becomes generated like everything else, or the clause goes.
% garden's resolution checked against the dataset: 5187x3361.
On a high resolution scene like Mip-NeRF~360 \emph{garden} ($5187\times3361$), the reference SSIM
already accounts for a tenth of training time at quarter and at half
resolution, and \SI{16}{\percent} at full resolution --- where it becomes the
second most expensive stage of the step, behind only backward rasterization.

In the standard formulation, SSIM statistics are computed at every pixel over a sliding $11\times11$ 
Gaussian window, so each pixel draws on up to $121$ neighbours. A workgroup producing a $16\times16$ output 
tile must stage a $26\times26$ patch of both the rendered and the ground-truth image.

In the backward pass, the gradient at a pixel is a blur of the per-pixel SSIM
derivatives which likewise reaches beyond the tile. Shared memory is private to
a workgroup, so these derivatives cannot be exchanged on chip. The forward pass
writes them to global memory as full-resolution derivative maps and the backward
pass reads them back with its own halo. The loss thus costs two dispatches
separated by a round trip.

We replace the sliding window with a non-overlapping one. Taking the window size
equal to the stride, and both equal to the $16\times16$ render tile, SSIM is
evaluated exactly once per tile from only the pixels of that tile, weighted
uniformly. Each pixel then contributes to exactly one statistic, which has two
consequences.

First, no pixel outside the tile is required. Second, since the tile score $M$
depends on a pixel only through those moments, its gradient is available in closed
form. No second convolution is
needed (original had a forward ssim and a backward ssim), and forward and backward fuse into a single dispatch in which no intermediate reaches global memory.

Lastly, a fixed tile partition places the window boundaries at the same pixels
at every iteration, so we offset the origin of the tile grid differently at each iteration,
stepping the phase in both axes. Each axis visits
all sixteen phases once every sixteen iterations.


% \gm{You should also explain the rationale behind your choices (you explained it very nicely our last meeting): neighbor pixel share a lots of characteristics due to spatial coherence, so in the intial framework, neighbour tiles provide redundant information for the gradient descent. Considering sparser sliding windows both improves efficiency and without compromising on performance (refer to result section).  }


==> sec/archive/method_draft_text.tex <==
% Method, rebuilt 2026-11-12 in the order of the figure board
% (https://claude.ai/artifact/7XSQ4QkfSHCuaMYaZBPwjJ). Text copied from the drafts named
% above each subsection; figures are the ones picked on the board. The previous method
% section is sec/archive/3_method_old.tex.
%
% \papfig{title}{file}: inputs a diagram float with its caption replaced by the title only
% (captions to be written by hand). The diagram files keep their long captions for the
% standalone previews.
\input{diagrams/bwd_ablation_macros}
\input{diagrams/projadam_ablation_macros}

\section{Method}
\label{sec:method}

% ---------------------------------------------------------------- Overview
% Text from sec/METHOD_DETAILS_DRAFT.tex, Overview
\subsection{Overview}
\label{sec:overview}
\papfig{Data movement per stage, ours}{diagrams/fig_pipeline}

The analysis gives three goals. Stages that scale with pixels need fewer (pixel, splat) pairs and fewer instructions per pair. Stages that scale with splats need fewer bytes. The sort needs fewer bits. \Cref{fig:overview,fig:pipeline} show the resulting pipeline. Two separations in the original disappear: key generation merges into projection, and projection backward merges into Adam. \Cref{tab:footprint} gives the data each stage moves and \cref{tab:ops} how it operates. On the RTX 3070 ladder in our Vulkan framework, each major change contributes as follows, in ms per step: pixel sampling 70.6 to 32.7, tile SSIM 32.7 to 32.0, the backward walk 32.0 to 12.5, fused keys 12.5 to 12.4, and the optimizer changes 12.4 to 11.3.

% ---------------------------------------------------------------- Directional Opacity and RGB
% Text from sec/CONE_COLOUR_DRAFT.tex
\subsection{Directional Opacity and RGB}
\label{sec:appearance}
\papfig{Cone opacity falloff}{diagrams/fig_alt_cone}
\papfig{Cone spawn rule}{diagrams/fig_alt_spawn}
\papfig{Cost of appearance per splat per view}{diagrams/table_appearance}

\paragraph{Direct colour.} Without view dependence, spherical harmonics reduce to degree 0, and the colour is an affine map of one coefficient per channel, clamped,
\begin{equation}
c_i=\max\bigl(0,\ C_0\,k_i+\tfrac12\bigr),\qquad C_0=\tfrac{1}{2\sqrt\pi}.
\label{eq:sh0}
\end{equation}
Projection evaluates this for each visible splat and writes $c_i$ to a colour buffer that the rasterizer reads. We store the colour itself,
\begin{equation}
c_i=(r_i,g_i,b_i),\qquad \frac{\partial L}{\partial(r_i,g_i,b_i)}=\frac{\partial L}{\partial c_i}.
\label{eq:direct}
\end{equation}
The arithmetic saved is small, three multiply-adds and a clamp. The larger gain is that projection no longer reads or writes colour: the rasterizers read the 12\,B parameter directly, and the backward pass copies the incoming gradient with no clamp mask. Against degree 0, projection drops from 48 to 40 registers and takes 10--15\% less time per splat. The colour is not clamped, which lets a splat subtract. Scaling the learning rate by $C_0$ keeps the optimisation trajectory of \cref{eq:sh0}.

\paragraph{Cone opacity.} Most implementations make colour depend on view, by default with degree-3 harmonics: 48 coefficients, 192\,B per splat, 16 basis functions of the view direction and 48 multiply-adds per view, and in the backward pass 48 gradients plus a gradient through the direction into the position (\cref{tab:appearance}). We instead let opacity depend on view. Each splat carries a unit axis $n_i$ and a slope $k_i$, 16\,B. With $w$ the unit direction from the splat to the camera, its opacity in that view is
\begin{equation}
\alpha'_i=\alpha_i\,f_i,\qquad f_i=\min\bigl(1,\ \max\bigl(0,\ 1-k_i\,(1-w\cdot n_i)\bigr)\bigr).
\label{eq:cone}
\end{equation}
The factor falls linearly from 1 on the axis and is exactly zero for $w\cdot n_i\le 1-1/k_i$, outside a cone of half-angle $\arccos(1-1/k_i)$ (\cref{fig:mech-cone}). A slope $k_i\le0$ gives $f_i=1$ from every direction. At $k_i=0$ the gradient on $k_i$ is still alive, so a splat can start omnidirectional and narrow continuously. Inside the ramp the derivatives are
\begin{equation}
\begin{gathered}
\frac{\partial\alpha'_i}{\partial n_i}=\alpha_i k_i\,w,\quad
\frac{\partial\alpha'_i}{\partial k_i}=-\alpha_i\,(1-w\cdot n_i),\\
\frac{\partial\alpha'_i}{\partial x_i}=-\frac{\alpha_i k_i}{\|o-x_i\|}\bigl(I-ww^{\top}\bigr)n_i,
\end{gathered}
\label{eq:cone-grad}
\end{equation}
with $o$ the camera centre, and zero outside it. After each Adam update $n_i$ is renormalised and $k_i$ clamped to $[0,4]$.

The factor costs one normalisation, one dot product, one multiply-add and a clamp. Projection evaluates it after reading the position, scale and opacity and before reading the rotation, and rejects the splat when $\alpha'_i\le1/255$. A splat outside its cone therefore costs 16\,B more than an off-screen one and produces no key, no sort entry and no rasterizer work. The rasterizers receive $\alpha'_i$ as they would receive $\alpha_i$ and are unchanged.

\paragraph{Other view-dependent splats.} Beta Splatting keeps a degree-0 colour and adds lobes, by default two per splat,
\begin{equation}
c_i(d)=\max\Bigl(0,\ c_{i,0}+\sum_{j=1}^{2}c_{ij}\,\max(0,\,d\cdot\mu_{ij})^{4e^{b_{ij}}}\Bigr),
\label{eq:sb}
\end{equation}
with each lobe axis $\mu_{ij}$ stored as two angles. That is 60\,B per splat, and per lobe and view two sine-cosine pairs, a power and an exponential. Universal Beta Splatting stores colour directly, as we do, and makes the kernel itself six-dimensional, three spatial and three angular dimensions. Every step it builds the $6\times6$ covariance of every splat and conditions it on the view direction, which yields a new mean, covariance and opacity per view, the opacity scaled by $\prod_{j=1}^{3}\bigl(1-\tanh y_j^2\bigr)^{\beta_j}$ with $y$ the whitened angular offset. This reads 280\,B and writes 196\,B per splat and view, for every splat, in frustum or not. Its opacity factor approaches zero but never reaches it, so no splat leaves the sort. Most other directional-opacity methods keep harmonic colour. VoD-3DGS adds a symmetric quadratic form in the view direction to the opacity logit, which can never be one-sided or zero. ARF gives about a tenth of the splats, added after training, a raised-cosine lobe that is exactly zero beyond a learned angle, but evaluates it outside the rasterizer, so a splat at zero still receives keys and is sorted. Scaffold-GS decodes colour, opacity and shape from anchor features with small networks, and discards generated splats whose opacity is not positive; its zero is exact and used, but it is found by running three networks over every visible anchor in every view. A soft opacity can only be culled by a threshold, which changes the image, or by a separate conservative bound, as N-DG does with three-sigma tests along random projections. An exact zero needs neither: the splat contributes nothing, so dropping it is lossless. The cone reaches that zero inside projection, from 16 bytes and one dot product, while the colour stays a plain parameter (\cref{tab:appearance}). It is also the least expressive: it cannot change a splat's colour with view, only whether and how strongly the splat is seen.
\todo{Quality comparison against SH2 at equal time; Beta Splatting/UBS numbers if we run them.}

\paragraph{Cone spawn.} Cones start from existing splats. A base splat keeps $k=-2$, frozen, and stays visible from every view. During training each splat accumulates the unit directions $v_j$ of the $V$ training views that have it in frustum, and the unit directions $e_j$ of the $m$ views in which it covers high-error pixels (at least one per megapixel). Their concentrations are the lengths of the means,
\begin{equation}
r_e=\Bigl\|\frac1m\sum_{j=1}^{m}e_j\Bigr\|,\qquad r_c=\Bigl\|\frac1V\sum_{j=1}^{V}v_j\Bigr\|,
\label{eq:spawn-r}
\end{equation}
both 1 when all directions agree. Every 500 steps from step 1500 to 15k, a base splat with $m\ge5$ and
\begin{equation}
1-r_e<\tfrac12\,(1-r_c)
\label{eq:spawn-test}
\end{equation}
has errors from a much narrower set of directions than the views that see it, and receives a copy with opacity $0.1$, axis and slope
\begin{equation}
n=\frac{\sum_j e_j}{\bigl\|\sum_j e_j\bigr\|},\qquad k=\min\Bigl(4,\ \frac{1}{2(1-r_e)+\frac14}\Bigr).
\label{eq:spawn-init}
\end{equation}
For directions spread evenly over a cap of half-angle $\theta$, the mean length is $r=(1+\cos\theta)/2$, so the cap edge is at $w\cdot n=2r_e-1$. \Cref{eq:spawn-init} puts the child's zero at $1-1/k=2r_e-1-\frac14$, a little outside that edge. All of this runs in device kernels over flat per-splat arrays: two float4 accumulators, one comparison and one copy per spawned splat.
\todo{Report gains on both the interleaved and a contiguous-arc split. Compare with Augmented Radiance Field, which already learns an exact-zero lobe: we claim the culling and spawning, not view-dependent opacity.}

% ---------------------------------------------------------------- Projection and Key Emission
% Text from sec/METHOD_DETAILS_DRAFT.tex, Projection + Key Generation
\subsection{Projection and Key Emission}
\label{sec:projkeys}
\papfig{Fused projection and keys, shared counter (ours)}{diagrams/fig_mech_projkeys_cursor}
\papfig{Projection and keys, original 3DGS}{diagrams/fig_mech_projkeys_inria}

\paragraph{Projection.}
\label{sec:proj}
Since this kernel is bound by DRAM, each change here removes bytes. Direct RGB colour replaces spherical harmonics, so the kernel no longer evaluates them and drops from 48 to 40 registers, and projection time per splat falls by 10--15\%. Dropping the radius and tile rectangle from the projected output and deriving the rectangle from fields already stored makes projection 9.1\% faster and key emission 6.3\% faster on garden, with all 40 test renders bit-identical. A visible splat now reads 60B where the original reads 236B.

We then address invisible splats. A conservative bound from the splat's position, scale, opacity and cone decides that a splat will receive no tile before its rotation is loaded, so a rejected splat reads 16--44B. Over 20 views on each of three trained models, projection results, keys and renders are byte-identical with the bound on and off. In training, the projection stage falls by 10.1\% on counter and 16.8\% on bonsai and garden, and the wall clock by 1.2--1.4\%, from one run each. PSNR was 0.005--0.09\,dB lower with the bound on in all five comparisons, which is inside run-to-run variation but consistently signed.

The memory order of the splats has almost no bearing here. With Morton reordering turned off the kernel gets faster (a ratio of 0.963), since projection streams the whole array anyway, while the stages that use the sorted lists slow down (\cref{sec:periodic}).

\paragraph{Key generation.}
\label{sec:keys}
We fuse key emission into projection. The original's second enumeration exists to give each splat a write offset, and that offset is needed only because the buffer is sized exactly. We drop both requirements. The key buffer has a grow-only capacity, and a block computes its own write offset without waiting for other blocks' data (\cref{fig:mech-keys}). A block publishes its count and reads those of its predecessors until it reaches a finished prefix, so it depends only on their counts and never on their writes. If capacity is exceeded, the step re-runs with a larger buffer.

We avoided the most direct design for a reason. A global cursor bumped by each warp through an atomic addition took 16.8\,ms per step in situ, against 0.3\,ms for the same scattered writes without it. We could not reproduce that cost outside the trainer, and the look-back design does not have it.

The unsorted keys are byte-identical to those of the two-pass design. The projection stage, which now includes emission, drops by 24--30\% (garden from 0.88\,ms to 0.73\,ms), and the wall clock by 1.9\% on average over five scenes. Around 30\% of that saving is the trimmed output of \cref{sec:proj}.

Tile overlap follows the exact ellipse, with a radius that shrinks with opacity, because a pair on a tile where the splat is invisible costs a sort entry and a list slot for nothing. On garden the result is 5.0 pairs per visible splat, with about 3\% of keys wasted.

% ---------------------------------------------------------------- Rasterization Forward
% Text from sec/METHOD_DETAILS_DRAFT.tex, Forward Rasterization
\subsection{Rasterization Forward}
\label{sec:fwd}

Testing each splat against all pixels of a tile spends arithmetic on pixels the splat may never reach. Each splat therefore computes a coarse mask of the subtiles it reaches, each warp maps to one subtile, and a warp reduces all the masks to a short ordered hit list. Lanes evaluate only that list (\cref{fig:mech-fwd}). Colour is held on chip as well, so that blending needs no global access and the original's 16B load per passing pair goes away.

The two changes only pay together. Colour in shared memory alone gives 1.05$\times$ and hit lists alone 1.07$\times$, but both give 1.22$\times$ (1.16--1.29$\times$ over 15 scenes), with bit-identical output. Each relieves one of the two limits found in \cref{sec:limits-fwd}, and easing one exposes the other. On the profiled view, instruction count and time both fall by 17\%, and the shared-memory pipe falls from 92\% to 79\% busy. In full training the stage is 1.22--1.26$\times$ faster and the wall clock 2.1--3.5\% lower, over four single runs.

This is one case in which we accept lower occupancy. The kernel holds 13312B of shared memory and six blocks per SM, against 7168B and eight in the original (\cref{tab:resources}). The additional blocks would only spend their time waiting for the global load we removed. Two alternatives did not survive: masking off the subtile test is 0.875$\times$, and two pixels per thread gives 1.13$\times$ alone, needs 53 registers, and does not combine with hit lists.

% ---------------------------------------------------------------- Loss (L1 + SSIM)
% Text from sec/LOSS_SECTION_DRAFT.tex
\subsection{Loss (L1 + SSIM)}
\label{sec:loss}
\papfig{Loss, original with fused-ssim}{diagrams/fig_mech_loss_inria}
\papfig{Loss, one block (ours)}{diagrams/fig_mech_loss_ours}

\paragraph{What the original computes.}
The original trains on $0.8\,\mathcal{L}_1 + 0.2\,(1-\mathrm{SSIM})$. SSIM compares the rendered and ground-truth images through local means, variances and covariance, taken under an $11\times11$ Gaussian window centred on every pixel. Its CUDA implementation~\cite{fusedssim} gives each block of $32\times32$ threads one pixel each (\cref{fig:mech-loss-inria}). Because the window reaches five pixels past the block, the block first copies a $42\times42$ patch of both images into on-chip shared memory, 1.7 times the pixels it produces. It then blurs five maps per channel, each in a pass over rows and a pass over columns of 11 taps. The gradient of a pixel depends on the SSIM derivatives of every window that covers it, which again reaches past the block. Blocks cannot share on-chip memory, so the first kernel writes three derivative maps per channel to global memory, and a second kernel reads them back with the same halo and blurs them once more. $\mathcal{L}_1$ is a separate PyTorch operation, and autograd adds the two gradients. In all, each pixel costs about 208\,B of global traffic and \pending{ncu: instructions per pixel}.


\paragraph{How it scales.}
None of this depends on the scene: the loss costs the same per pixel whatever the image shows. At low resolution it is a small part of a step, but every other stage grows with the number of splats, while the loss grows with the number of pixels. \Cref{fig:loss-scaling} times it on \emph{garden} from one eighth to full resolution, \pending{0.27 to 17.4\,MP: x ms to y ms}. At full resolution it is \SI{16}{\percent} of a training step on the RTX~3090, second only to backward rasterization.


\paragraph{Why it is slow.}
Each streaming multiprocessor (SM) of the GPU runs threads in groups of 32 called warps, and keeps up to 48 warps resident so that while some wait on memory, others compute. How many fit is set by three budgets per SM: 65\,536 registers, up to 100\,KB of shared memory, and 1\,536 threads. \Cref{tab:loss-invoice} itemizes what one block of the original asks for. Its staged patches and blur scratch take 20.5\,KB of shared memory. Each of its 1\,024 threads holds 46 registers, 49\,152 in all. A second block would need more registers than the SM has, so each SM holds one block, 32 warps, on the RTX~3070 and on the RTX~4090 alike. Those 32 warps also move in lockstep: every blur pass ends at a barrier where the whole block waits, \pending{ncu: achieved occupancy x\%}.


\paragraph{Ours.}
We take SSIM over non-overlapping $16\times16$ blocks with a uniform window (\cref{fig:mech-loss-ours}). Under a uniform window a block's SSIM depends on its pixels only through five sums per channel, so the gradient of a pixel has a closed form in those sums and the pixel's own values. Nothing outside the block is needed and no second kernel runs. Each thread loads one pixel; each warp adds its 32 pixels by exchanging registers; the eight warps meet in 576\,B of shared memory; each thread then writes its pixel's $\mathcal{L}_1$ and SSIM gradient. The loss value itself is never computed, since training only needs the gradient. At 40 registers for 256 threads, six blocks fit on an SM, all 48 warps (\cref{tab:loss-invoice}). Per pixel the kernel moves 36\,B and executes \pending{ncu: instructions per pixel}. The block grid is offset differently every step, cycling through 16 positions on each axis, so block edges never stay on the same pixels.


\paragraph{With strided sampling.}
The loss runs on the packed image of the current sampling phase (\cref{sec:sampling}), so a block holds $16\times16$ samples spread over $32\times32$ screen pixels. It is the size of a render tile, but not aligned with one: the loss grid moves every step and the render grid does not. The two changes save separately. Sampling divides the pixels per step by four; the uniform window lowers the cost of each pixel. On the packed image the original loss takes \pending{x ms} and ours \pending{y ms} (\cref{fig:loss-scaling}).


\paragraph{Is a tiled window a good stand-in?}
The uniform window is an approximation of SSIM, not SSIM itself, so we evaluate with the standard Gaussian SSIM on full-resolution renders. \Cref{fig:ssim-quality} trains the same model with each loss, both under strided sampling. Over the seven Mip-NeRF~360 scenes the two curves stay within 0.002 throughout, ending at 0.858 and 0.859 at 50k steps, while the loss stage falls from 2.31\,ms to 0.28\,ms per step on the RTX~3070. These runs used our earlier Vulkan implementation; the kernel is the same algorithm. \pending{prior art for uniform-window, non-overlapping SSIM not yet checked}

% ---------------------------------------------------------------- Rasterization Backward
% Text from sec/BWD_ABLATION_DRAFT.tex
\subsection{Rasterization Backward}
\label{sec:backward}
\papfig{Backward ablation schedules}{diagrams/fig_bwd_ablation}
\papfig{Backward ablation}{diagrams/table_bwd_ablation}

\Cref{fig:bwd-ablation} and \cref{tab:bwd-ablation} take the backward pass from
gsplat's kernel to ours in six steps. Every row runs inside our pipeline on the
same forward outputs of \bwdAblScenes{} trained scenes, so only the backward
differs; the gsplat and Taming rows are ports of the official kernels, changed
only where our pixel layout and buffers force it. Each part of the figure shows
what a thread is and, in a strip of time steps, what it handles at each step.

\paragraph{gsplat: a thread is a pixel.}
Each of a tile's 256 threads owns one pixel. All of them step through the tile's
splats together, back to front, each starting from its pixel's final
transmittance and dividing every splat's contribution back
out~\cite{ye2024gsplat}. A splat's gradient is therefore spread over the pixels'
threads, and at every step each warp sums its 32 lanes' terms and issues nine
atomic additions.

\paragraph{Taming: a thread is a splat.}
Taming-3DGS gives the thread to the splat~\cite{mallick2024taming}, so a splat's
gradient accumulates in one thread's registers and is written once. The tile's
splats are cut into buckets of 32, one warp each. A lane steps across the tile's
256 pixels one behind the lane before it, and the pixel's state is handed from
lane to lane. Buckets run independently of one another, which requires the state
of every pixel at the start of every bucket: the forward saves it, and the first
lane of each warp loads it. This is \bwdAblStepTaming{} faster than gsplat.

\paragraph{A: the tile's block owns the pixel state.}
We keep a thread per splat but give each tile one block of 128 threads that
holds the state of its 256 pixels in shared memory. The block takes the splats
in order from the front, where the state is known ($T = 1$, no colour), in
batches of up to 128 that follow one another. The forward saves nothing and the
backward loads nothing. This is the largest step, \bwdAblStepA{}.

\paragraph{B: lean pair arithmetic.}
The schedule is that of A; a (splat, pixel) pair costs less. The pixel keeps the
transmittance and one scalar in place of the three-channel colour, and a pair
adds to moments of the pixel offset, to which the splat's opacity and conic are
applied once at the end (\bwdAblStepB{}).

\paragraph{C: one warp per splat, one chunk per step.}
A splat now gets a whole warp, and the warp's 32 lanes are the 32 pixels of one
$8{\times}4$ chunk of the tile, so a step updates a chunk and the splat's
gradient is summed across the lanes in registers. Depth order is kept by a rule
local to the splat: it enters a chunk when the splat before it has left that
chunk. With four warps, four splats are in flight on different chunks
(\bwdAblStepC{}).

\paragraph{D: skip chunks unreached by the splat.}
A splat tests its footprint against the eight chunks and walks only those it
reaches. It still waits on the splat before it, so on the example the schedule
barely shortens.

\paragraph{E: wait per chunk.}
With the reached chunks known, a splat waits only for the earlier splats that
reach the same chunk, and splats with disjoint footprints run side by side.

\paragraph{What the steps are worth.}
The example schedules shrink from \bwdAblToyStepsC{} steps (C) to
\bwdAblToyStepsD{} (D) and \bwdAblToyStepsE{} (E), but the
measured gains of D and E are \bwdAblStepD{} and \bwdAblStepE{}: counting steps
overstates them, because a chunk a splat does not reach is rejected cheaply and
finding the reached chunks has its own cost. End to end the backward is
\bwdAblSpeedE{} faster than gsplat's, and most of that is structural: who owns
the pixel state (A) and what a warp is (C). D and E together add
\bwdAblStepCE{}; C needs neither the chunk test nor the per-chunk counters.

% ---------------------------------------------------------------- Projection Backward and Adam
% Text from sec/PROJADAM_DRAFT.tex
\subsection{Projection Backward and Adam}
\label{sec:adam}
\papfig{Projection backward and Adam ablation}{diagrams/table_projadam_ablation}
\papfig{Share of splats visible per view}{diagrams/fig_visibility}

After the rasterizer, every splat that was drawn holds nine screen-space gradients. This stage carries them back through the projection to the parameters and takes an Adam step. It does little arithmetic and moves many bytes, so its cost is set by how many bytes each splat moves, and by how many splats it touches.

\paragraph{What is published.}
Three ideas for this stage exist, spread over different systems; none has all three (\cref{tab:projadam-ablation}).
\emph{Skipping unseen splats.} Taming-3DGS~\cite{mallick2024taming} and gsplat~\cite{ye2024gsplat} offer an Adam that reads a per-splat visibility flag and leaves a splat with no tile in the view untouched; the 3DGS reference code later adopted Taming's version. In all three it is opt-in. It runs after autograd, so the gradient buffers are still cleared for every splat and the activation backward still runs over every splat.
\emph{One kernel.} VkSplat~\cite{vksplat} runs the projection backward and Adam in the same thread, recomputing the projection from the parameters it loads anyway, so no gradient buffer is written or read back. It updates every splat, giving the unseen ones a zero gradient.
\emph{Compact moments.} LichtFeld~\cite{lichtfeld} also fuses Adam into its projection backward and keeps both moments in 16 bits per parameter (8 for the higher SH bands). It too updates every splat. Brush~\cite{brussee2024brush} shares one second moment across a splat's SH coefficients.

\paragraph{What we do.}
We combine the three: one kernel per splat that recomputes the projection, returns after reading the splat's tile count when the splat touched no tile, and stores both moments as a bf16 pair. None of the three ideas is ours. The combination is not in any of the systems above, and it matters because each idea alone leaves a large cost in place (\cref{tab:projadam-ablation}). Skipping in a separate Adam still clears and differentiates every splat; fusing without skipping moves every unseen splat's parameters and moments. On average a view sees \paAblVisible{} of the splats (\cref{fig:visibility}), so the unseen ones dominate. Inside a fused kernel the skip is complete: an unseen splat costs a 4-byte read and nothing else.

The skip is the same test gsplat and Taming use, with three differences. The flag is the projection's tile count rather than a positive radius, so splats removed by the cone or too faint to draw are also skipped. There is one launch and one thread per splat, instead of one launch per parameter group and one thread per parameter element. And because there are no gradient buffers, nothing is cleared for an unseen splat.

\paragraph{Measured.}
\Cref{tab:projadam-ablation} starts from gsplat with its sparse Adam on (\paAblgsplatms\,ms on our 15 trained scenes, SH degree 3, rebuilt inside our pipeline) and adds one change per row. Moving the projection backward and Adam into one kernel, keeping the skip, gives \paAblAms\,ms (\paAblASpeed): no gradient buffer is written or read back, and an unseen splat no longer pays for clearing and differentiating its buffers. Storing the moments as bf16 pairs gives \paAblBms\,ms. The last row is our model change, RGB colour with the cone instead of SH, at \paAblCms\,ms (\paAblCSpeed). For reference, VkSplat's kernel, which fuses but updates every splat, takes \paAblVkSplatms\,ms, and LichtFeld's design, which adds 16-bit moments to it, \paAblLichtFeldms\,ms. bf16 moments do not measurably change quality (\cref{tab:projadam-bf16}).

\todo{Add a LichtFeld bib entry; decide whether the RGB + cone row belongs here or in the appearance section.}

% Flush the method floats before Results (float-only pages otherwise lose single-column figures in this build).
\clearpage

% ---- Overview as it was before the 2026-11-16 merge with Nicholas's text (Claude-written)
% Overview rewritten again 2026-11-16 at Nicholas's request (Claude-written, NOT YET VETTED):
% motivation + setup for the stages (what each is bound by, which take the time, how each
% scales with splats, resolution and GPU), with little about our changes. The stage-list
% sentence and the VkSplat sentence are from his old overview. Numbers come from
% tables/stage_shift_macros.tex (figsrc/build_stage_shift.py: vanilla VkSplat b3ad2b0,
% upstream MCMC config, garden, RTX 3070 + baseline on a Vast.ai RTX 4090, its own per-pass timer
% over steps 9000-9300). GPU specs: vendor figures as in figsrc/build_gpu_specs.py.
% \input{tables/stage_shift_macros}
% Table "Per-stage timings" (tables/table_stage_shift) is issued in sec/1_intro.tex so it lands on page 2 with the data-movement figure.

% The stages of a step in 3DGS training are projection, key generation, sort, rasterization, loss, rasterization backward, projection backward, optimizer and densification. They differ in what they run over: projection, projection backward, the optimizer and densification run once per splat; key generation and sort run once per splat--tile pair; rasterization, the loss and rasterization backward run once per pixel. Each kind is bound by something different, so each scales with something different, and which stage dominates a step depends on the scene, the resolution and the GPU. \Cref{tab:stage-shift} times each stage of an unmodified VkSplat~\cite{vksplat} training step on garden with an RTX~3070: VkSplat's MCMC configuration with 1M splats on images capped at 1600 pixels wide (\ShiftMPBase\,MP), the cap the reference 3DGS implementation applies by default, as the baseline, then three times the splats and the full-resolution images (\ShiftResPixels times the pixels). Each cell is the stage's share of the step's GPU time. We also timed VkSplat's recommended configuration (1M splats, \ShiftMPQuarter\,MP images) on an RTX~3070 and an RTX~4090; the per-stage speedups are given below.

% \paragraph{Per-splat stages.} One thread per splat loads the splat's parameters, transforms them, and writes the result back. There is little arithmetic per byte, so these stages are bound by DRAM bandwidth. Their time follows the splat count and nothing else: with three times the splats, projection takes \ShiftSplatsProj$\times$ as long and projection backward with Adam \ShiftSplatsProjBwdAdam$\times$, while \ShiftResPixels times the pixels leaves both unchanged. Projection backward with Adam reads every splat's parameters and gradients and reads and writes both Adam moments, and with degree-3 spherical harmonics most of those bytes are colour. It is \ShiftPctBaseProjBwdAdam\% of the baseline step and \ShiftPctSplatsProjBwdAdam\% at 3M splats, close behind rasterization backward (\ShiftPctSplatsRastBwd\%).

% \paragraph{Per-pair stages.} Key generation writes one key per splat--tile pair, and sort orders them. Both are memory-bound passes over the pair list, whose length grows with the splat count and also with resolution, since a splat spans more tiles as the image grows. They stay a small part of the step (at most \ShiftPctResKeys\% and \ShiftPctResSort\% at full resolution).

% \paragraph{Per-pixel stages.} Rasterization walks each tile's depth-sorted splats for every pixel of the tile, evaluating and blending each splat that overlaps it. This is arithmetic on data staged in shared memory, so it is compute-bound, and its cost grows with the pixel count times the number of splats overlapping each pixel. Rasterization backward replays the blend and accumulates each pixel's contribution into the gradients of the splats it saw; many pixels contribute to the same splat, so the gradients need a reduction across pixels. It is the largest stage of the baseline step (\ShiftPctBaseRastBwd\%). The loss depends on the images only: an L1 term and SSIM, whose Gaussian windows make several passes over the rendered and ground-truth images. The ground-truth image also has to be copied to the GPU every step. With \ShiftResPixels times the pixels, rasterization backward takes \ShiftResRastBwd$\times$ as long, the loss \ShiftResLoss$\times$ and the upload \ShiftResUpload$\times$; rasterization backward is then \ShiftPctResRastBwd\% of the step and the loss \ShiftPctResLoss\%.

% \paragraph{Hardware.} The RTX~4090 has \(2.3\times\) the memory bandwidth of the RTX~3070 (1008 vs.\ 448\,GB/s) but \(4.1\times\) its FP32 throughput (82.6 vs.\ 20.3\,TFLOPS). On VkSplat's recommended configuration, projection and projection backward with Adam run \ShiftGpuProj$\times$ and \ShiftGpuProjBwdAdam$\times$ faster, matching the bandwidth ratio, while rasterization forward and backward run \ShiftGpuRastFwd$\times$ and \ShiftGpuRastBwd$\times$ faster and the loss \ShiftGpuLoss$\times$. The ground-truth upload does not speed up at all (\ShiftGpuUpload$\times$): both cards copy over the same PCIe~4.0~x16 link, so on the 4090 it is \ShiftPctGpuUpload\% of the step. The faster the GPU, the larger the share of the step that goes to stages bound by memory or by the host link rather than by compute.

% No single stage dominates across these settings, so speeding up one stage mostly moves the bottleneck to another. Our target, full-resolution training on consumer GPUs, sits in the high-resolution column, where the per-pixel stages take most of the step, but the per-splat stages grow back as splat counts rise. We therefore go through every stage, in the order a step runs them (\cref{sec:appearance,sec:projkeys,sec:fwd,sec:loss,sec:bwd,sec:adam}). \Cref{fig:pipeline} shows the data each stage reads and writes in our pipeline, and \cref{tab:stage_times} gives its per-stage times. Our codebase is built on top of VkSplat's released work~\cite{vksplat}.


% ---- Rasterization Forward as it was before the 2026-11-17 rewrite (Nicholas's text)
% Text from Desktop/Bare Necessity.docx (2026-11-13), "Rasterization Fwd", prepended.
% The last sentence is unfinished in the docx and is kept as written.
% The motivation for splats to be sorted to tiles is for tile level depth sorting instead of a global sort. But in forward rasterization stage, which is also tile-based, there is room for even more preprocessing so the splats of a tile are only rasterized by the subtiles they cover.

% Current implementations map a block which is some number of warps to every tile, with each warp handling a share of the pixels of that tile. For example, 8 warps (32 threads each) making 1 block (256 threads) can each take 1 subtile ($8{\times}4=32$ pixels).

% But splats do not cover all subtiles within a tile. Thus we first preprocess splats

% \label{sec:sampling}
% \papfig{Strided pixel sampling}{diagrams/fig_strided_sampling}
% \gm{it is not very clear to me on how this section is linked to the tile SIMM Section !? Maybe you could clarify ?}
% Turbo-GS~\cite{dhiman2024turbogs} first introduced ``Dilated Rendering'', where a systematically strided subset of full-resolution images is used to train instead of using downsampled images. We adopt this idea and make some implementation changes, but our implementation does not quite have the dilation element and so we will refer to it as ``Strided Pixel Sampling''. 

% We hypothesize that as training resolution rises, neighboring pixels may
% contribute increasingly similar gradients to the Gaussians they cover, so a
% strided subset of a full-resolution image may supervise competitively at a lower cost. 

% We evaluate two variants. The first, \emph{\nicefrac{1}{2} stride}, splits each
% training image into two half-density images in a checkerboard-like pattern. The
% second, \emph{\nicefrac{1}{4} stride}, splits it into
% four, on a $2{\times}2$ grid, so that each step supervises $WH/4$ pixels---the
% same per-iteration pixel budget as half-resolution (which has a quarter of the pixels), but with four phases covering the full-resolution image over four steps.

% We highlight the differences between our implementation and Turbo-GS's. Firstly, instead of reducing the number of threads per workgroup, we increase the tile size so that the number of pixels rendered per tile per iteration is unchanged. A tile (which is usually $16{\times}16$ in both full and half-resolution training) covers a $32{\times}16$ screen rectangle under \nicefrac{1}{2} stride and $32{\times}32$ under \nicefrac{1}{4} stride. The \nicefrac{1}{4} stride scheme and half resolution therefore render the same number of pixels per tile over the same screen area
% (\cref{fig:sampling}). Not having a reduced thread count has a positive impact on performance, and also reduces the number of tiles.

% Secondly, we do this for the entire training, with no progressive resolution schedule. Each training image is first split into two or four separate images prior to training and stays that way throughout. This is to avoid loading the full image at each step. Total memory usage (for holding training images) stays unchanged.

% Lastly, Turbo-GS applies a lattice-matched blur for compensation, which we do not. 

% Because the stride is regular, the implementation stays cheap: tile lists, keys and sort stages are
% phase-independent and hence require no change. Per-pixel buffers can be sized
% down to $WH/2$ and $WH/4$ for the two- and four-phase schemes respectively, and
% the split training images are compacted the same way. 



==> sec/archive/table_pipeline_profile.tex <==
% Stock-pipeline stage profile -- generated by figsrc/build_pipeline_profile.py
\begin{table}[t]\centering\small
\setlength{\tabcolsep}{2.6pt}
\setlength{\fboxsep}{1.5pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l r r@{}}
\toprule
Stage & Time/step & Share of total time \\
\midrule
Projection & 0.3\,ms & 0.4\% \\
Key emission~\colorbox[HTML]{FFF3A8}{(\cref{sec:keys-stage})} & 1.2\,ms & 1.7\% \\
Sort & 1.5\,ms & 2.1\% \\
Rasterize forward~\colorbox[HTML]{FFF3A8}{(\cref{sec:sampling})} & 3.5\,ms & 5.0\% \\
Loss (SSIM)~\colorbox[HTML]{FFF3A8}{(\cref{sec:tile-ssim})} & 8.6\,ms & 12.2\% \\
Rasterize backward~\colorbox[HTML]{FFF3A8}{(\cref{sec:backward})} & 53.2\,ms & 75.5\% \\
Optimizer & 1.3\,ms & 1.9\% \\
Other & 0.8\,ms & 1.1\% \\
\midrule
Total & 70.6\,ms & 100\% \\
\bottomrule
\end{tabular*}
\input{sec/archive/table_pipeline_profile_caption}
\label{tab:pipeline-profile}
\end{table}


==> sec/archive/table_pipeline_profile_caption.tex <==
\caption{Per-stage timings for baseline training step. Measured on RTX~3070 over all 15 scenes at full-resolution. Rasterize backward implementation measured here is gsplat.}


==> sec/archive/table_provenance.tex <==
% SHELVED 2026-11-20 (Nicholas): was Sec. 3.9 "Summary" (\subsection{Summary}\label{sec:provenance}), removed from the paper.
% To restore: \input{sec/archive/table_provenance} in sec/3_method.tex + \inlinecap{sec/archive/table_provenance} in sec/captions.tex.
% Provenance of every change, by stage (Sec. 3.9). Claude-written 2026-11-20, NOT YET VETTED.
% Hand-written, no generator. Fact-check sources (2026-11-20 session):
%   UBS RGB colour: own code read (table_appearance header, UBS 1b502a4).
%   ARF exact-zero lobe, keys still emitted: AuGS_Code 57cca00 + RESULTS_ARCHIVE/cone_runs/reports/Cone opacity prior art.md.
%   RoofGS (arXiv 2608.15785v1, 16 Aug 2026, RENDERING only): "combining preprocessing, tile duplication, and key-value
%     generation into a single kernel ... shared-memory prefix sums and a single global atomic operation per block";
%     also a 32-bit tile|quantized-depth key. How its buffer is sized is not stated.
%   VkSplat 32-bit key: project page "compresses tile-depth keys to 32 bits (14 bits tile ID + 18 bits depth)".
%   VkSplat subtile masks + colour in shared: upstream code (alphablend_shader.slang, SHARED_STRUCT float3 rgb), not in its paper.
%   Warp-Level Culling (Yang, Drettakis, Bernstein, PACMCGIT 9(4) 2026): warps subdivide a tile and cull non-overlapping
%     splats, data rearranged for shared memory; code = fork of Faster-GS. Whether it compacts a list: not confirmed.
%   Local-GS (arXiv 2606.16566, rendering): "culling stage that discards warps with no contribution".
%   HiGS: per-warp popc-compacted queue, inference only (gsplat experimental MacroTileRasterize.cu).
%   Turbo-GS v3 (9 May 2026): "For each iteration we randomly sample one offset"; tile-Gaussian pairs from the
%     downsampled image.
%   ByteSplat (arXiv 2610.02851): S3IM "applied independently within each image tile" so the loss fuses with rasterization.
%   VkSplat project page: fused kernel for the gradient of L1+SSIM; SSIM formulation itself unchanged.
%   fused-ssim: sliding 11x11 Gaussian window, forward + backward kernels (fig_mech_loss_inria, checked vs 1272e21).
%   LiteGS: arXiv 2503.01199 Sec 3.1/App A.1 + raster.cu (warp per tile on one splat, no checkpoints, scanline sums).
%   VkSplat per-splat bwd without checkpoints, credits Taming: upstream b3ad2b0.
%   Sparse Adam: gsplat selective_adam.py "one of the two optimizers mentioned in the Taming3DGS paper";
%     Faster-GS also credits it to Mallick et al.
%   Fused proj-bwd + Adam: VkSplat project page "merged into a single kernel pass"; LichtFeld 393aa42 code.
%   Compact moments: LichtFeld 393aa42 code (16-bit, 8-bit for higher SH).
%   FastGS score: arXiv 2511.04283 (K=10 sampled views).
%   Host-memory GT: Inria 3DGS --data_device cpu.
% Rows marked "Ours" = no prior found in the checks above; the scalar colour state and per-chunk waits were not
% searched beyond the backward survey in memory (perchunk prior art, 2026-11-20).
\begin{table*}[t]
    \centering
    % CAPTION (hand-edited, kept when the table is regenerated) begin
    \caption[Where each change comes from]{Where each change comes from.\ {\normalfont
    Adopted: used as in the cited work. Adapted: the cited work has the idea, we change it as noted. Ours: not found in prior work.}}
    % CAPTION end
    \footnotesize
    \renewcommand{\arraystretch}{1.08}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}l p{4.6cm} p{5.6cm} l p{4.2cm}@{}}
    \toprule
    Stage & Change & Prior work & Status & What is ours \\
    \midrule
    \multirow{4}{*}{Appearance}
      & Flat RGB color instead of SH & RGB color in UBS~\cite{liu2026ubs}; equals SH degree 0 & Adopted & --- \\
      & Cone opacity: axis $\mathbf n$, linear falloff $k$ & Exact-zero view lobe in ARF~\cite{yang2026arf} (SH3, ${\sim}10\%$ of splats) & Adapted & Form, on every cone splat, with RGB \\
      & Cull splats outside their cone & Back-face culling; ARF still emits keys & Ours & Culling before key emission \\
      & Spawn cone splats from high-error views & --- & Ours & All \\
    \midrule
    \multirow{4}{*}{\shortstack[l]{Projection\\and keys}}
      & Direct RGB, no color pass & Follows from flat RGB & Ours & All \\
      & Frustum/opacity cull before loading rotation and cone & Frustum culling in 3DGS~\cite{kerbl20233dgs} & Adapted & Load order \\
      & One-pass projection and key emission, one atomic per wave & RoofGS~\cite{luo2026roofgs}: same fusion, per block, rendering only & Adapted & Training; buffer sized from peak history \\
      & 32-bit keys (tile, truncated depth) & VkSplat~\cite{vksplat}; also RoofGS~\cite{luo2026roofgs} & Adopted & --- \\
    \midrule
    \multirow{4}{*}{\shortstack[l]{Forward\\raster}}
      & $8{\times}4$ subtile masks per warp & VkSplat~\cite{vksplat}; warp-level culling~\cite{yang2026warpcull,luo2026localgs} & Adopted & --- \\
      & Per-warp hit lists & HiGS~\cite{higs}, inference only & Adapted & Training forward, subtile scale \\
      & Color staged in shared memory & VkSplat~\cite{vksplat}; \cite{yang2026warpcull} & Adopted & --- \\
      & Strided pixel sampling, $2{\times}2$ & Turbo-GS~\cite{dhiman2024turbogs}: random offset, pairs at low res. & Adapted & Cycled offset; full-res.\ footprints; $32{\times}32$ tiles \\
    \midrule
    \multirow{2}{*}{Loss}
      & Non-overlapping tile SSIM, closed-form gradient, one dispatch & \texttt{fused-ssim}~\cite{fusedssim}: sliding window, two passes; ByteSplat~\cite{wu2026bytesplat}: per-tile S3IM & Ours & Uniform window on the render tile, gradient without a second pass \\
      & Tile grid offset each step & --- & Ours & All \\
    \midrule
    \multirow{5}{*}{\shortstack[l]{Backward\\raster}}
      & No checkpoints, one pixel state per tile & 3DGS, gsplat~\cite{ye2024gsplat}, VkSplat~\cite{vksplat}, LiteGS~\cite{liao2026litegs}; checkpoints from Taming~\cite{mallick2024taming} & Adopted & --- \\
      & A warp per splat & LiteGS~\cite{liao2026litegs}: one warp per tile on one splat & Adapted & Over 32-pixel chunks, several splats in flight \\
      & Skip unreached chunks, wait per chunk & --- & Ours & All \\
      & Scalar color state $a$ & --- & Ours & All \\
      & Splat constants applied once; \texttt{exp2} & LiteGS~\cite{liao2026litegs} sums w.r.t.\ quadratic coefficients & Adapted & Moments per splat over chunks \\
    \midrule
    \multirow{3}{*}{\shortstack[l]{Projection\\bwd + Adam}}
      & Sparse Adam (skip unseen splats) & Taming-3DGS~\cite{mallick2024taming}; gsplat~\cite{ye2024gsplat} & Adopted & --- \\
      & Projection backward fused with Adam & VkSplat~\cite{vksplat}, LichtFeld~\cite{lichtfeld} & Adopted & --- \\
      & Compact (bf16) moments & LichtFeld~\cite{lichtfeld} (16/8-bit) & Adopted & Choice of bf16 \\
    \midrule
    \multirow{2}{*}{Densification}
      & Error-count score & FastGS~\cite{fastgs} & Adopted & --- \\
      & Score from training renders & FastGS renders sampled views & Ours & All \\
    \midrule
    Data & Ground truth in host memory, uploaded per step & 3DGS~\cite{kerbl20233dgs} (\texttt{data\_device cpu}) & Adopted & Triple buffering \\
    \bottomrule
    \end{tabular}
    \label{tab:provenance}
\end{table*}


==> tables/captions/table1_comparison.tex <==
\caption[\captitle{tables/table1_comparison}]{\usecap{tables/table1_comparison}}
% caption text: sec/captions.tex


==> tables/captions/table1_comparison_otherinfo.tex <==
\caption{Main comparison, with other info for ours}


==> tables/captions/table_ablation_ladder_minus.tex <==
\caption{Ablation ladder}


==> tables/captions/table_bwd_impl.tex <==
\caption{Measured Rasterization Backward implementations}


==> tables/captions/table_ck4_vs_r2.tex <==
\caption{\nicefrac{1}{4} strided pixel sampling and half-resolution training comparison over seven Mip-NeRF~360 scenes}


==> tables/captions/table_cone_class.tex <==
\caption{Peak memory and model size per scene}


==> tables/captions/table_gpu_specs.tex <==
\caption{GPUs used in this paper.}


==> tables/captions/table_stage_share.tex <==
\caption{Share of a training step by stage on an RTX~3070}


==> tables/captions/table_stage_shift.tex <==
% gm: "not sure this Table is the best to come first... interesting, but in the intro, should be a highlight of paper results."
% Addressed 2026-11-16: moved from the intro to the method overview (sec:overview).
\caption[\captitle{tables/table_stage_shift}]{\usecap{tables/table_stage_shift}}
% caption text: sec/captions.tex


==> tables/captions/table_stage_times.tex <==
\caption[\captitle{tables/table_stage_times}]{\usecap{tables/table_stage_times}}
% caption text: sec/captions.tex


==> tables/table1_comparison_otherinfo.tex <==
% TRIAL generated by figsrc/build_comparison_otherinfo.py from tables/table1_comparison.tex + figsrc/data/cone_class.json -- do not edit
% Row order = slowest to fastest on the 4090, as on the artifact page.
\begin{table*}[t]\centering\scriptsize
\setlength{\tabcolsep}{2.6pt}
\begin{tabular}{@{}l rrrrr @{\hskip4pt\vrule width0.4pt\hskip4pt} rrrr @{\hskip5pt\vrule width0.9pt\hskip5pt} rrrrr @{\hskip4pt\vrule width0.4pt\hskip4pt} rrrr@{}}
\toprule
 & \multicolumn{9}{c}{Mip-NeRF 360 (7 scenes)} & \multicolumn{9}{c}{Tanks \& Temples 4K (8 scenes)} \\
\cmidrule(r{2pt}){2-10}\cmidrule(l{2pt}){11-19}
Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Splats & MB & 3060 & 3070 & 3090 & 4090 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Splats & MB & 3060 & 3070 & 3090 & 4090 \\
\midrule
Mip-Splatting & 28.83 & \cellcolor{rankone}0.866 & \cellcolor{rankone}0.234 & 3.59M & 906 & -- & -- & -- & 103m 43s & 23.34 & \cellcolor{rankthree}0.813 & \cellcolor{ranktwo}0.251 & 2.71M & 682 & -- & -- & -- & 87m 23s \\
Speedy-Splat & 27.57 & 0.824 & 0.366 & 0.20M & 51 & -- & -- & 88m 59s & \phantom{0}70m \phantom{0}7s & 22.92 & 0.778 & 0.371 & 0.16M & 39 & -- & -- & 79m 20s & 64m \phantom{0}0s \\
Taming-3DGS & 28.26 & 0.840 & 0.328 & 0.62M & 153 & -- & -- & 53m 15s & \phantom{0}25m \phantom{0}9s & 23.62 & 0.787 & 0.349 & 0.33M & 82 & -- & -- & 39m 33s & 19m 14s \\
DashGaussian & 28.57 & 0.853 & 0.272 & 2.14M & 531 & -- & -- & 42m 20s & \phantom{0}19m 50s & 24.03 & 0.807 & 0.283 & 1.60M & 398 & -- & -- & 30m \phantom{0}0s & 15m 13s \\
Faster-GS & 28.45 & 0.851 & 0.293 & 1.92M & 453 & 48m \phantom{0}8s & 33m \phantom{0}3s & 19m 50s & \phantom{0}16m 31s & 23.49 & 0.807 & 0.280 & 1.59M & 375 & 50m \phantom{0}4s & 30m 39s & 19m 30s & 11m 58s \\
VkSplat & 28.39 & 0.850 & 0.297 & 2.35M & 556 & 40m 59s & 27m \phantom{0}3s & 16m 20s & \phantom{0}10m 32s & 23.14 & 0.803 & 0.291 & 1.79M & 423 & 37m 44s & 23m 25s & 13m 51s & \phantom{0}8m \phantom{0}7s \\
LiteGS & \cellcolor{rankone}29.30 & \cellcolor{ranktwo}0.863 & \cellcolor{rankthree}0.256 & 0.99M & 246 & \cellcolor{ranktwo}34m \phantom{0}8s & \cellcolor{ranktwo}23m 54s & 15m 38s & \cellcolor{rankthree}\phantom{00}8m 17s & \cellcolor{rankone}24.84 & \cellcolor{ranktwo}0.819 & \cellcolor{rankthree}0.252 & 0.99M & 246 & \cellcolor{ranktwo}32m \phantom{0}2s & \cellcolor{rankthree}22m 23s & 14m 54s & \phantom{0}8m \phantom{0}5s \\
LichtFeld & \cellcolor{ranktwo}29.14 & \cellcolor{ranktwo}0.863 & \cellcolor{ranktwo}0.252 & 1.00M & 248 & 38m 35s & 28m 30s & \cellcolor{rankthree}14m 52s & \cellcolor{ranktwo}\phantom{00}8m \phantom{0}7s & \cellcolor{rankthree}24.21 & \cellcolor{rankone}0.821 & \cellcolor{rankone}0.236 & 1.00M & 248 & 38m 46s & 26m 16s & \cellcolor{rankthree}13m 50s & \cellcolor{rankthree}\phantom{0}7m 23s \\
FastGS & 28.36 & 0.847 & 0.299 & 0.54M & 134 & \cellcolor{rankthree}37m 17s & \cellcolor{rankthree}25m \phantom{0}1s & \cellcolor{ranktwo}14m 11s & \phantom{00}8m 22s & 23.31 & 0.797 & 0.308 & 0.43M & 107 & \cellcolor{rankthree}34m \phantom{0}8s & \cellcolor{ranktwo}21m 12s & \cellcolor{ranktwo}12m \phantom{0}0s & \cellcolor{ranktwo}\phantom{0}6m 57s \\
\midrule
\textbf{Ours (30k)} & \cellcolor{rankthree}28.96 & \cellcolor{rankthree}0.855 & 0.263 & 1.57M & 95 & \cellcolor{rankone}\phantom{0}6m 25s & \cellcolor{rankone}\phantom{0}4m 24s & \cellcolor{rankone}\phantom{0}2m 56s & \cellcolor{rankone}\phantom{00}1m 29s & \cellcolor{ranktwo}24.35 & \cellcolor{rankthree}0.813 & 0.258 & 1.71M & 112 & \cellcolor{rankone}\phantom{0}6m 37s & \cellcolor{rankone}\phantom{0}4m 36s & \cellcolor{rankone}\phantom{0}3m \phantom{0}6s & \cellcolor{rankone}\phantom{0}1m 38s \\
\midrule
\textit{Ours (30k)} & \multicolumn{4}{r@{\hskip8.4pt}}{File size 95\,MB (max 179\,MB)} & \multicolumn{4}{l@{\hskip5pt\vrule width0.9pt\hskip5pt}}{\sbox0{Host memory}\makebox[\wd0][l]{Host memory} 9.42\,GB (max 13.5\,GB)} & \multicolumn{4}{r@{\hskip8.4pt}}{File size 112\,MB (max 160\,MB)} & \multicolumn{4}{l}{\sbox0{Host memory}\makebox[\wd0][l]{Host memory} 10.3\,GB (max 12.6\,GB)} \\
\textit{other info} & \multicolumn{4}{r@{\hskip8.4pt}}{35\% cone, 65\% base splats} & \multicolumn{4}{l@{\hskip5pt\vrule width0.9pt\hskip5pt}}{\sbox0{Host memory}\makebox[\wd0][l]{GPU memory} 0.96\,GB (max 1.76\,GB)} & \multicolumn{4}{r@{\hskip8.4pt}}{59\% cone, 41\% base splats} & \multicolumn{4}{l}{\sbox0{Host memory}\makebox[\wd0][l]{GPU memory} 1.11\,GB (max 1.46\,GB)} \\
\bottomrule
\end{tabular}
\input{tables/captions/table1_comparison_otherinfo}
\label{tab:main_comparison}
\end{table*}


==> tables/table_ablation_ladder_minus.tex <==
% Ablation ladder (removal direction) -- generated by figsrc/build_ladder.py
% Ours at the top; each row removes one more component going down.
\begin{table*}[t]\centering\scriptsize
\setlength{\tabcolsep}{1.7pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l c @{\hskip5pt\vrule width0.9pt\hskip5pt} rrrr @{\hskip4pt\vrule width0.4pt\hskip4pt} rrr @{\hskip5pt\vrule width0.9pt\hskip5pt} rrrr @{\hskip4pt\vrule width0.4pt\hskip4pt} rrr@{}}
\toprule
\multicolumn{2}{@{}l@{}}{} & \multicolumn{7}{c}{Mip-NeRF 360 (7 scenes)} & \multicolumn{7}{c}{Tanks \& Temples 4K (8 scenes)} \\
\cmidrule(lr{2pt}){3-9}\cmidrule(l{2pt}){10-16}
Configuration & Iters & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & VRAM & RTX3060 & RTX3070 & RTX3090 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & VRAM & RTX3060 & RTX3070 & RTX3090 \\
\midrule
\textbf{Ours} & \textbf{60k} & \textbf{28.80} & \textbf{0.858} & \textbf{0.244} & \textbf{2.53\,GB} & \textbf{21m 10s} & \textbf{13m 58s} & \textbf{\phantom{0}8m 13s} & \textbf{23.89} & \textbf{0.807} & \textbf{0.259} & \textbf{1.78\,GB} & \textbf{16m \phantom{0}4s} & \textbf{11m 12s} & \textbf{\phantom{0}7m \phantom{0}3s} \\
w/o Fused Keys \& Opt & 60k & 28.80 & 0.858 & 0.243 & 2.47\,GB & 22m 58s & 15m 33s & \phantom{0}9m \phantom{0}5s & 23.86 & 0.807 & 0.260 & 1.69\,GB & 17m \phantom{0}2s & 12m 12s & \phantom{0}7m 32s \\
w/o Rast. Bwd & 60k & 28.83 & 0.858 & 0.243 & 2.47\,GB & 53m 29s & 36m 40s & 19m 39s & 23.89 & 0.807 & 0.260 & 1.68\,GB & 46m 41s & 30m 42s & 18m \phantom{0}9s \\
w/o Tile SSIM & 50k & 28.64 & 0.859 & 0.259 & 2.26\,GB & 45m 32s & 28m 54s & 16m 52s & 23.80 & 0.810 & 0.266 & 1.73\,GB & 40m 43s & 27m 36s & 16m 17s \\
w/o Pixel Sampling & 30k & 27.99 & 0.837 & 0.335 & 1.80\,GB & 53m 19s & 34m 18s & 19m 35s & 23.09 & 0.796 & 0.315 & 1.60\,GB & 57m \phantom{0}6s & 37m 13s & 21m 40s \\
\bottomrule
\end{tabular}}
\input{tables/captions/table_ablation_ladder_minus}
\label{tab:ablation_ladder}
\end{table*}


==> tables/table_bwd_impl.tex <==
% Backward implementations at a trained state -- generated by figsrc/build_bwd_impl.py
% Do not edit by hand; edit the generator and re-run.
\begin{table}[t]\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rr r@{}}
\toprule
Backward Implementation & Forward & Backward & Total \\
\midrule
Front-to-Back, shared state \textbf{(ours)} & 3.7\,\si{\milli\second} & 15.0\,\si{\milli\second} & 25.1\,\si{\milli\second} \\
Back-to-Front, autodiff & 3.7\,\si{\milli\second} & 19.7\,\si{\milli\second} & 29.7\,\si{\milli\second} \\
Front-to-Back, registers & 3.6\,\si{\milli\second} & 22.0\,\si{\milli\second} & 31.9\,\si{\milli\second} \\
Checkpointed segments & 4.4\,\si{\milli\second} & 22.9\,\si{\milli\second} & 33.6\,\si{\milli\second} \\
\midrule
Per-Gaussian buckets \textit{\scriptsize(Taming-3DGS)} & 4.6\,\si{\milli\second} & 16.9\,\si{\milli\second} & 28.0\,\si{\milli\second} \\
Per-pixel reverse \textit{\scriptsize(3DGS/gsplat)} & 3.7\,\si{\milli\second} & 58.9\,\si{\milli\second} & 68.9\,\si{\milli\second} \\
\bottomrule
\end{tabular*}
\input{tables/captions/table_bwd_impl}
\label{tab:bwd_impl}
\end{table}


==> tables/table_ck4_vs_r2.tex <==
% Strided sampling vs half resolution, generated by figsrc/build_sampling.py
% Do not edit by hand; edit the generator and re-run.
\begin{table}[t]\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l c rrr r@{}}
\toprule
Sampling & Iters & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & RTX3070 \\
\midrule
Half-resolution & 80k & 28.11 & 0.840 & 0.270 & 14m 11s \\
\textbf{\nicefrac{1}{4} strided pixels (ours)} & \textbf{80k} & \textbf{28.88} & \textbf{0.858} & \textbf{0.243} & \textbf{17m 47s} \\
\bottomrule
\end{tabular}}
\input{tables/captions/table_ck4_vs_r2}
\label{tab:ck4_vs_r2}
\end{table}


==> tables/table_cone_class.tex <==
% generated by figsrc/build_cone_class.py from figsrc/data/cone_class.json -- do not edit
\begin{table}[t]\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Scene & \shortstack[r]{CPU RAM\\(GB)} & \shortstack[r]{VRAM\\(GB)} & \shortstack[r]{Splats\\(M)} & \shortstack[r]{Cones\\(\%)} & \shortstack[r]{File\\(MB)} \\
\midrule
bicycle & 12.9 & 1.91 & 2.91 & 34 & 179 \\
bonsai & 7.8 & 0.55 & 0.78 & 28 & 47 \\
counter & 6.6 & 0.52 & 0.69 & 44 & 44 \\
garden & 13.5 & 1.58 & 2.43 & 38 & 151 \\
kitchen & 7.5 & 0.77 & 1.05 & 48 & 67 \\
room & 8.3 & 0.59 & 0.72 & 30 & 43 \\
stump & 9.2 & 1.45 & 2.28 & 23 & 136 \\
caterpillar & 11.1 & 1.10 & 1.76 & 63 & 117 \\
family & 12.6 & 1.19 & 1.76 & 45 & 111 \\
francis & 11.3 & 0.88 & 1.14 & 58 & 75 \\
horse & 3.3 & 0.78 & 1.11 & 74 & 75 \\
ignatius & 11.4 & 1.53 & 2.55 & 42 & 160 \\
lighthouse & 11.4 & 1.31 & 1.61 & 76 & 110 \\
train & 10.5 & 1.18 & 1.73 & 67 & 115 \\
truck & 10.9 & 1.51 & 2.13 & 43 & 134 \\
\bottomrule
\end{tabular*}
\input{tables/captions/table_cone_class}
\label{tab:cone-class}
\end{table}


==> tables/table_cone_cull.tex <==
% generated by figsrc/build_cone_cull.py from figsrc/data/cone_cull_split -- do not edit
\begin{table}[t]
    \centering
    % CAPTION (hand-edited, kept when the table is regenerated) begin
    \caption[Distribution of splats and culling]{Distribution of splats and culling}
    % old (2026-11-20): \caption[Distribution of splats and culling]{Where a view's splats go.\ {\normalfont
    % Per view, as a share of all splats in the model, mean over the views of each scene and then over the \coneCullScenes{} scenes. Outside the view: covers no tile even with its cone opened.}}
    % old: \caption{Where a view's splats go}
    % CAPTION end
    \footnotesize
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l r r r@{}}
        \toprule
        \% of all splats & Base (\%) & Cone (\%) & All (\%) \\
        \midrule
        Splats in the model & 52.4 & 47.6 & 100 \\
        Outside the view & 33.9 & 16.3 & 50.2 \\
        Culled by the cone & --- & 16.8 & 16.8 \\
        \midrule
        Drawn & 18.5 & 14.5 & 33.0 \\
        \bottomrule
    \end{tabular*}
    \label{tab:cone_cull}
\end{table}


==> tables/table_gpu_specs.tex <==
% GPU specifications -- generated by figsrc/build_gpu_specs.py
% Vendor part data, not measurements. Do not edit by hand; edit the
% generator and re-run. FP32 and bandwidth are derived from the primary
% specs in that script and checked against the published figures.
\begin{table}[!b]\centering\small
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rrrr@{}}
\toprule
GPU & FP32 (TFLOPS) & VRAM & Bandwidth & TDP (W) \\
\midrule
RTX3060 & 12.7 & 12\,GB & 360\,GB/s & 170 \\
RTX3070 & 20.3 & 8\,GB & 448\,GB/s & 220 \\
RTX3090 & 35.6 & 24\,GB & 936\,GB/s & 350 \\
RTX4090 & 82.6 & 24\,GB & 1008\,GB/s & 450 \\
\bottomrule
\end{tabular*}
\input{tables/captions/table_gpu_specs}
\label{tab:gpus}
\end{table}


==> tables/table_loss_stage.tex <==
% Per-step SSIM-loss cost -- generated by figsrc/build_loss_stage.py
% Bare tabular: it lives inside a minipage, the caption is on the figure*.
{\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}l rr rr@{}}
\toprule
 & \multicolumn{2}{c}{Loss Stage Time} & \multicolumn{2}{c}{Total Train Time} \\
\cmidrule(lr){2-3}\cmidrule(l){4-5}
Loss & RTX~3070 & RTX~3090 & RTX~3070 & RTX~3090 \\
\midrule
Full SSIM & 2.31\,ms & 1.23\,ms & 34.7\,ms & 20.2\,ms \\
Tiled SSIM & 0.28\,ms & 0.17\,ms & 36.7\,ms & 19.6\,ms \\
\bottomrule
\end{tabular}}


==> tables/table_quality_ablation.tex <==
% generated by figsrc/build_quality_ablation.py from figsrc/data/ablation_std.jsonl
\begin{table}[t]\centering\footnotesize
\caption[\captitle{tables/table_quality_ablation}]{\usecap{tables/table_quality_ablation}}
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rrrrr@{}}
\toprule
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & MB & RTX3070 \\
\midrule
Ours & 26.48 & 0.832 & 0.287 & 118 & \phantom{0}4m 29s \\
\midrule
w/o strided sampling & 26.50 & 0.832 & 0.286 & 117 & 15m \phantom{0}4s \\
w/o Tile SSIM & 26.34 & 0.833 & 0.290 & 112 & \phantom{0}5m 11s \\
w/o RGB + cone (SH3) & 25.99 & 0.829 & 0.293 & 278 & \phantom{0}4m 23s \\
\bottomrule
\end{tabular*}
\label{tab:quality_ablation}
\end{table}


==> tables/table_sd_all.tex <==
% generated by figsrc/build_stage_detail.py (all_table) from figsrc/data/stage_detail_time.jsonl,
% stage_detail_keys_sh0_time.jsonl (projection and keys) + stage_detail_ncu/
\begin{table}[t]\centering\footnotesize
% CAPTION (hand-edited, kept when the table is regenerated) begin
% 2026-11-20 Claude-written, NOT YET VETTED
\caption[Changes within each stage]{Changes within each stage.\ {\normalfont Each block goes from the standard implementation (first row) to ours, each row adding one change to the row above. Kernels, instructions and DRAM traffic per training step (Nsight Compute) and GPU memory on garden; stage time on an RTX~3070, mean over \sdNumScenes{} scenes, and its speedup over the block's first row. Backward rasterization and projection backward with Adam have their own tables (\cref{tab:bwd-ablation,tab:projadam-ablation}).}}
% CAPTION end
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rrrrrr@{}}
\toprule
 & Kernels & Instr.\ & DRAM & VRAM & Time & Speedup \\
 & & & traffic & & & \\
 & & (M) & (MB) & (MB) & (ms) & \\
\midrule
\multicolumn{7}{@{}l}{\textit{Projection and keys}} \\
\quad 3DGS: 2 passes, SH0 & 5 & 69 & 339 & 1{,}288 & 0.85 & 1.00$\times$ \\
\quad + one fused pass & 2 & 70 & 273 & 1{,}172 & 0.66 & 1.27$\times$ \\
\quad + direct RGB & 2 & 68 & 221 & 1{,}092 & 0.57 & 1.49$\times$ \\
\quad\textbf{+ early reject (ours)} & \textbf{2} & \textbf{63} & \textbf{175} & \textbf{1{,}092} & \textbf{0.48} & \textbf{1.74$\times$} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Sort}} \\
\quad 64-bit keys (3DGS) & 9 & 95 & 788 & 1{,}184 & 1.81 & 1.00$\times$ \\
\quad\textbf{32-bit keys (ours)} & \textbf{7} & \textbf{62} & \textbf{362} & \textbf{1{,}092} & \textbf{0.81} & \textbf{2.22$\times$} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Rasterization forward}} \\
\quad No subtile masks & 1 & 1{,}023 & 152 & 1{,}092 & 2.73 & 1.00$\times$ \\
\quad + subtile masks (VkSplat) & 1 & 877 & 152 & 1{,}092 & 2.38 & 1.15$\times$ \\
\quad + shared colour & 1 & 859 & 152 & 1{,}092 & 2.27 & 1.20$\times$ \\
\quad\textbf{+ hit lists (ours)} & \textbf{1} & \textbf{682} & \textbf{152} & \textbf{1{,}092} & \textbf{1.93} & \textbf{1.41$\times$} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Loss}} \\
\quad \texttt{fused-ssim}, $11{\times}11$ & 5 & 349 & 1{,}207 & 1{,}492 & 2.22 & 1.00$\times$ \\
\quad\textbf{Tile SSIM (ours)} & \textbf{1} & \textbf{57} & \textbf{156} & \textbf{1{,}092} & \textbf{0.28} & \textbf{8.05$\times$} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Pixels per step (fwd, loss, bwd)}} \\
\quad Full image & 12 & 11{,}496 & 3{,}417 & 1{,}092 & 32.33 & 1.00$\times$ \\
\quad\textbf{Strided, 1 in 4 (ours)} & \textbf{3} & \textbf{2{,}875} & \textbf{853} & \textbf{1{,}092} & \textbf{8.20} & \textbf{3.94$\times$} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Appearance (whole step, same splats)}} \\
\quad SH degree 3, no cone & 13 & 3{,}156 & 2{,}634 & 2{,}214 & 11.19 & 1.00$\times$ \\
\quad\textbf{RGB + cone opacity (ours)} & \textbf{13} & \textbf{3{,}053} & \textbf{1{,}709} & \textbf{1{,}092} & \textbf{10.07} & \textbf{1.11$\times$} \\
\bottomrule
\end{tabular*}
\label{tab:sd_all}
\end{table}


==> tables/table_sd_bwd.tex <==
% generated by figsrc/build_stage_detail.py from figsrc/data/stage_detail_time.jsonl + stage_detail_ncu/
\begin{table}[t]\centering\footnotesize
\caption[\captitle{tables/table_sd_bwd}]{\usecap{tables/table_sd_bwd}}
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l rrrrrrrrr@{}}
\toprule
 & threads & regs & shared & occu- & issue & instr. & VRAM & time & slow- \\
 & /block & /thread & (KB) & pancy & slots & (M) & (MB) & (ms) & down \\
\midrule
gsplat & 256 & 40 & 10.0 & 95\% & 43\% & 4262 & 1{,}092 & 22.01 & 3.68$\times$ \\
Taming-3DGS & 32 & 58 & 0.8 & 33\% & 65\% & 4870 & 1{,}712 & 19.42 & 3.22$\times$ \\
Ours & \textbf{128} & \textbf{48} & \textbf{9.0} & \textbf{83\%} & \textbf{84\%} & \textbf{2135} & \textbf{1{,}092} & \textbf{6.00} & \textbf{1.00$\times$} \\
\bottomrule
\end{tabular*}
\label{tab:sd_bwd}
\end{table}


==> tables/table_stage_share.tex <==
% generated by figsrc/build_stage_times.py
\begin{table*}[t]\centering\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l c c c c c c c rr@{}}
\toprule
Ablation & Proj.\ Fwd & Sort & Raster Fwd & Loss & Raster Bwd & Proj.\ Bwd + Adam & Other & Step & vs Ours \\
\midrule
\textbf{{\name} (Ours)} & \textbf{\makebox[1.9em][r]{4\%}} & \textbf{\makebox[1.9em][r]{7\%}} & \textbf{\makebox[1.9em][r]{17\%}} & \textbf{\makebox[1.9em][r]{3\%}} & \textbf{\makebox[1.9em][r]{55\%}} & \textbf{\makebox[1.9em][r]{6\%}} & \textbf{\makebox[1.9em][r]{8\%}} & \textbf{\makebox[1.05em][r]{8}.\makebox[1.05em][l]{98}\,ms} &  \\
w/o Fused Keys, Sort & \cellcolor{rankone}\makebox[1.9em][r]{6\%} & \cellcolor{rankone}\makebox[1.9em][r]{15\%} & \makebox[1.9em][r]{15\%} & \makebox[1.9em][r]{2\%} & \makebox[1.9em][r]{49\%} & \makebox[1.9em][r]{6\%} & \makebox[1.9em][r]{7\%} & \makebox[1.05em][r]{9}.\makebox[1.05em][l]{98}\,ms & 1.11$\times$ \\
w/o Raster Fwd, Sampl. & \makebox[1.9em][r]{1\%} & \makebox[1.9em][r]{2\%} & \cellcolor{rankone}\makebox[1.9em][r]{26\%} & \makebox[1.9em][r]{3\%} & \makebox[1.9em][r]{64\%} & \makebox[1.9em][r]{2\%} & \makebox[1.9em][r]{2\%} & \makebox[1.05em][r]{30}.\makebox[1.05em][l]{12}\,ms & 3.35$\times$ \\
w/o Tile SSIM & \makebox[1.9em][r]{4\%} & \makebox[1.9em][r]{6\%} & \makebox[1.9em][r]{14\%} & \cellcolor{rankone}\makebox[1.9em][r]{19\%} & \makebox[1.9em][r]{45\%} & \makebox[1.9em][r]{5\%} & \makebox[1.9em][r]{7\%} & \makebox[1.05em][r]{10}.\makebox[1.05em][l]{38}\,ms & 1.16$\times$ \\
w/o Raster Bwd & \makebox[1.9em][r]{2\%} & \makebox[1.9em][r]{3\%} & \makebox[1.9em][r]{7\%} & \makebox[1.9em][r]{1\%} & \cellcolor{rankone}\makebox[1.9em][r]{81\%} & \makebox[1.9em][r]{3\%} & \makebox[1.9em][r]{3\%} & \makebox[1.05em][r]{21}.\makebox[1.05em][l]{69}\,ms & 2.42$\times$ \\
w/o Fused Adam & \makebox[1.9em][r]{4\%} & \makebox[1.9em][r]{6\%} & \makebox[1.9em][r]{15\%} & \makebox[1.9em][r]{2\%} & \makebox[1.9em][r]{46\%} & \cellcolor{rankone}\makebox[1.9em][r]{20\%} & \makebox[1.9em][r]{7\%} & \makebox[1.05em][r]{10}.\makebox[1.05em][l]{49}\,ms & 1.17$\times$ \\
w/o RGB + Cone & \cellcolor{rankone}\makebox[1.9em][r]{6\%} & \makebox[1.9em][r]{7\%} & \makebox[1.9em][r]{15\%} & \makebox[1.9em][r]{3\%} & \makebox[1.9em][r]{47\%} & \cellcolor{rankone}\makebox[1.9em][r]{14\%} & \makebox[1.9em][r]{9\%} & \makebox[1.05em][r]{8}.\makebox[1.05em][l]{76}\,ms & 0.98$\times$ \\
\midrule
w/o All Changes & \makebox[1.9em][r]{1\%} & \makebox[1.9em][r]{2\%} & \makebox[1.9em][r]{8\%} & \makebox[1.9em][r]{10\%} & \makebox[1.9em][r]{72\%} & \makebox[1.9em][r]{6\%} & \makebox[1.9em][r]{1\%} & \makebox[1.05em][r]{77}.\makebox[1.05em][l]{54}\,ms & 8.63$\times$ \\
\bottomrule
\end{tabular*}
\input{tables/captions/table_stage_share}
\label{tab:stage_share}
\end{table*}


==> tables/table_stage_shift.tex <==
% Table 1 (stage shift). Body HAND-EDITED on Overleaf: do not rerun figsrc/build_stage_shift.py over it (it rewrites the body; only the caption below is kept). Caption: edit inline here.
\begin{table}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    % CAPTION (hand-edited, kept when the table is regenerated) begin
    \caption[Per-stage training time]{Per-stage training time.\ {\normalfont
    One training step of VkSplat (garden, RTX~3070) under different configurations.}}
    % old caption (2026-11-20): The bottleneck stage moves with the configuration. GPU time (ms) of each stage in one
    % training step of unmodified VkSplat on garden on an RTX~3070, excluding the ground-truth upload, which can be
    % overlapped with the step, in ms with its share of the step. The first column is the baseline (1600-pixel-wide
    % images, 1M splats). The second column triples the splats and the third trains at full resolution; each changes
    % only the factor in bold, and grey values are the baseline's. \rankbox{ranktwo}{Highlighted} cells show the stages
    % whose share grow most. More splats grow the per-splat stages and more pixels the per-pixel stages, so the
    % bottleneck moves with the configuration and no single stage dominates.
    % CAPTION end
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccc@{}}
        \toprule
         & Baseline & More Splats & Full Resolution \\
        \midrule
        Resolution & 1600$\times$1037 & \textcolor{dgmute}{1600$\times$1037} & \textbf{5187$\times$3361} \\
        \# Splats & 1M & \textbf{3M} & \textcolor{dgmute}{1M} \\
        % GPU & RTX 3070 & \textcolor{dgmute}{RTX 3070} & \textcolor{dgmute}{RTX 3070} \\
        \midrule
        Projection & 0.6 (5\%) & 1.9 (7\%) & 0.6 (1\%) \\
        Key emission & 0.3 (3\%) & 0.6 (2\%) & 2.3 (4\%) \\
        Sort & 0.5 (4\%) & 1.1 (4\%) & 2.0 (4\%) \\
        Rast.\ forward & 1.0 (8\%) & 2.1 (7\%) & 6.3 (11\%) \\
        Loss & 1.2 (9\%) & 1.2 (4\%) & {\setlength{\fboxsep}{1pt}\colorbox{rankthree}{\textbf{14.7 (26\%)}}} \\
        Rast.\ backward & 5.4 (42\%) & 11.1 (38\%) & 26.1 (47\%) \\
        Proj.\ bwd + Adam & 3.5 (28\%) & {\setlength{\fboxsep}{1pt}\colorbox{rankthree}{\textbf{10.3 (36\%)}}} & 3.4 (6\%) \\
        Densify (MCMC) & 0.2 (2\%) & 0.6 (2\%) & 0.2 (0\%) \\
        \midrule
        Total GPU time & 12.9 & 29.0 & 55.7 \\
        \bottomrule
    \end{tabular*}
    \label{tab:stage-shift}
\end{table}

